Cutting Plane Approaches for the Robust Kidney Exchange Problem

Renal patients which have a willing but incompatible donor can decide to participate in a kidney exchange program (KEP). The goal of a KEP is to identify sets of such incompatible pairs that can exchange donors, leading to compatible transplants for each recipient. There is significant uncertainty involved in this process, as planned transplants may be canceled for a plethora of reasons. It is therefore crucial to take into account failures while planning exchanges. In this paper, we consider a robust variant of this problem with recourse studied in the literature that takes into account vertex failures, i.e., withdrawing donors and/or recipients. This problem belongs to the class of defender-attacker-defender (DAD) models. We propose a cutting plane method for solving the attacker-defender subproblem based on two commonly used mixed-integer programming formulations for kidney exchange. Our results imply a running time improvement of one order of magnitude compared to the state-of-the-art. Moreover, our cutting plane methods can solve a large number of previously unsolved instances. Furthermore, we propose a new practical policy for recourse in KEPs and show that the robust optimization problem concerning this policy is tractable for small to mid-size KEPs in practice.

==> Tables/AggregatedLifting/aggr_lifting_table-cyc3-method1-policy1.tex <==
% generated by paper_generate_aggr_lifting_table.sh 3 s c 1
\begin{table}[htbp]
  \begin{scriptsize}
    \caption{Comparison of the cut-CC method with and without lifting for maximum cycle length 3 and different chain lengths, for the Full Recourse policy.}
    \label{tab:aggrlifting_cyc3-method1-policy1}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrr@{}}\toprule
       & \multicolumn{4}{c}{with lifting} & \multicolumn{4}{c}{without lifting}\\
      \cmidrule{2-5} \cmidrule{6-9}
      \#vertices & \#opt & time & \#att. & \#sub & \#opt & time & \#att. & \#sub \\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 2}\\
       20 &  120 & 0.1 & 2.8 & 8.0 &  120 & 0.1 & 3.0 & 10.0\\
       50 &  120 & 7.3 & 5.1 & 41.7 &  120 & 17.8 & 5.3 & 113.1\\
      100 &  120 & 132.3 & 5.6 & 104.5 &  107 & 329.8 & 5.6 & 217.2\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 3}\\
       20 &  120 & 0.2 & 2.8 & 8.4 &  120 & 0.3 & 3.0 & 10.8\\
       50 &  120 & 29.6 & 5.4 & 45.4 &  119 & 50.6 & 5.5 & 126.6\\
      100 &  88 & 1382.8 & 5.9 & 98.6 &  60 & 1765.7 & 5.9 & 215.8\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 4}\\
       20 &  120 & 0.8 & 2.9 & 8.8 &  120 & 0.8 & 2.9 & 11.3\\
       50 &  118 & 247.9 & 5.4 & 50.7 &  111 & 376.3 & 5.8 & 127.8\\
      100 &  8 & 3364.8 & 5.5 & 66.6 &  4 & 3490.3 & 2.7 & 22.6\\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{table}


==> Tables/AggregatedLifting/aggr_lifting_table-cyc3-method1-policy2.tex <==
% generated by paper_generate_aggr_lifting_table.sh 3 s c 2
\begin{table}[htbp]
  \begin{scriptsize}
    \caption{Comparison of the cut-CC method with and without lifting for maximum cycle length 3 and different chain lengths, for the FSE policy.}
    \label{tab:aggrlifting_cyc3-method1-policy2}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrr@{}}\toprule
       & \multicolumn{4}{c}{with lifting} & \multicolumn{4}{c}{without lifting}\\
      \cmidrule{2-5} \cmidrule{6-9}
      \#vertices & \#opt & time & \#att. & \#sub & \#opt & time & \#att. & \#sub \\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 2}\\
       20 &  120 & 0.5 & 3.4 & 9.2 &  120 & 0.5 & 3.4 & 11.8\\
       50 &  108 & 169.7 & 11.3 & 92.2 &  107 & 222.7 & 11.5 & 149.4\\
      100 &  45 & 2023.3 & 11.7 & 151.9 &  41 & 2082.3 & 8.1 & 71.1\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 3}\\
       20 &  120 & 1.6 & 3.6 & 10.8 &  120 & 1.8 & 3.8 & 15.1\\
       50 &  80 & 683.2 & 10.4 & 74.1 &  81 & 764.1 & 11.1 & 112.7\\
      100 &  16 & 3219.8 & 5.8 & 26.0 &  18 & 3152.0 & 12.7 & 112.0\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 4}\\
       20 &  120 & 4.6 & 3.7 & 11.0 &  120 & 4.4 & 3.6 & 13.7\\
       50 &  37 & 1790.4 & 10.4 & 57.3 &  39 & 1784.6 & 11.0 & 68.3\\
      100 &  1 & 3590.4 & 1.5 & 5.0 &  1 & 3591.7 & 1.2 & 2.8\\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{table}


==> Tables/AggregatedLifting/aggr_lifting_table-cyc3-method2-policy1.tex <==
% generated by paper_generate_aggr_lifting_table.sh 3 s p 1
\begin{table}[htbp]
  \begin{scriptsize}
    \caption{Comparison of the cut-PICEF method with and without lifting for maximum cycle length 3 and different chain lengths, for the Full Recourse policy.}
    \label{tab:aggrlifting_cyc3-method2-policy1}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrr@{}}\toprule
       & \multicolumn{4}{c}{with lifting} & \multicolumn{4}{c}{without lifting}\\
      \cmidrule{2-5} \cmidrule{6-9}
      \#vertices & \#opt & time & \#att. & \#sub & \#opt & time & \#att. & \#sub \\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 2}\\
       20 &  120 & 0.2 & 2.7 & 7.9 &  120 & 0.1 & 2.8 & 9.3\\
       50 &  120 & 11.6 & 5.3 & 35.4 &  118 & 24.5 & 5.2 & 102.6\\
      100 &  119 & 269.4 & 5.7 & 84.8 &  103 & 488.6 & 6.2 & 199.0\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 3}\\
       20 &  120 & 0.3 & 2.8 & 7.8 &  120 & 0.3 & 2.9 & 10.0\\
       50 &  120 & 27.4 & 4.9 & 40.8 &  118 & 35.7 & 5.1 & 97.5\\
      100 &  114 & 507.0 & 5.6 & 79.2 &  93 & 955.3 & 6.1 & 195.9\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 4}\\
       20 &  120 & 0.5 & 2.7 & 7.7 &  120 & 0.4 & 2.9 & 10.8\\
       50 &  120 & 48.7 & 4.9 & 43.0 &  117 & 67.8 & 5.1 & 110.8\\
      100 &  106 & 820.4 & 5.6 & 67.4 &  81 & 1465.5 & 5.8 & 192.6\\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{table}


==> Tables/AggregatedLifting/aggr_lifting_table-cyc3-method2-policy2.tex <==
% generated by paper_generate_aggr_lifting_table.sh 3 s p 2
\begin{table}[htbp]
  \begin{scriptsize}
    \caption{Comparison of the cut-PICEF method with and without lifting for maximum cycle length 3 and different chain lengths, for the FSE policy.}
    \label{tab:aggrlifting_cyc3-method2-policy2}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrr@{}}\toprule
       & \multicolumn{4}{c}{with lifting} & \multicolumn{4}{c}{without lifting}\\
      \cmidrule{2-5} \cmidrule{6-9}
      \#vertices & \#opt & time & \#att. & \#sub & \#opt & time & \#att. & \#sub \\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 2}\\
       20 &  120 & 0.7 & 3.4 & 8.5 &  120 & 0.7 & 3.4 & 11.4\\
       50 &  95 & 374.0 & 10.0 & 53.0 &  95 & 347.7 & 9.8 & 82.5\\
      100 &  40 & 2297.2 & 6.7 & 69.7 &  36 & 2486.5 & 7.1 & 33.8\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 3}\\
       20 &  120 & 1.9 & 3.6 & 9.8 &  120 & 1.8 & 3.6 & 12.7\\
       50 &  70 & 877.4 & 9.5 & 42.5 &  73 & 932.0 & 10.3 & 77.6\\
      100 &  16 & 2931.9 & 2.0 & 6.7 &  14 & 2992.4 & 1.0 & 2.1\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 4}\\
       20 &  120 & 2.6 & 3.8 & 11.0 &  120 & 2.8 & 3.9 & 15.4\\
       50 &  54 & 1088.5 & 8.2 & 44.7 &  56 & 1203.4 & 9.4 & 65.7\\
      100 &  6 & 3303.9 & 1.0 & 2.2 &  6 & 3340.8 & 1.0 & 2.4\\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{table}


==> Tables/AggregatedLifting/aggr_lifting_table-cyc4-method1-policy1.tex <==
% generated by paper_generate_aggr_lifting_table.sh 4 s c 1
\begin{table}[htbp]
  \begin{scriptsize}
    \caption{Comparison of the cut-CC method with and without lifting for maximum cycle length 4 and different chain lengths, for the Full Recourse policy.}
    \label{tab:aggrlifting_cyc4-method1-policy1}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrr@{}}\toprule
       & \multicolumn{4}{c}{with lifting} & \multicolumn{4}{c}{without lifting}\\
      \cmidrule{2-5} \cmidrule{6-9}
      \#vertices & \#opt & time & \#att. & \#sub & \#opt & time & \#att. & \#sub \\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 2}\\
       20 &  120 & 0.3 & 2.8 & 8.8 &  120 & 0.4 & 2.9 & 13.0\\
       50 &  120 & 33.4 & 5.3 & 45.0 &  118 & 78.5 & 5.5 & 151.3\\
      100 &  83 & 1350.5 & 4.9 & 77.7 &  52 & 2295.3 & 5.8 & 265.3\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 3}\\
       20 &  120 & 0.4 & 2.9 & 9.9 &  120 & 0.5 & 3.0 & 13.4\\
       50 &  120 & 71.2 & 5.2 & 51.9 &  117 & 136.9 & 5.3 & 162.4\\
      100 &  54 & 2390.0 & 4.8 & 74.5 &  30 & 2979.7 & 8.8 & 337.6\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 4}\\
       20 &  120 & 0.9 & 2.9 & 9.5 &  120 & 1.0 & 2.9 & 13.7\\
       50 &  115 & 325.7 & 5.0 & 48.4 &  103 & 523.7 & 5.2 & 144.9\\
      100 &  7 & 3465.9 & 3.8 & 59.1 &  2 & 3531.8 & 0.8 & 13.9\\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{table}


==> Tables/AggregatedLifting/aggr_lifting_table-cyc4-method1-policy2.tex <==
% generated by paper_generate_aggr_lifting_table.sh 4 s c 2
\begin{table}[htbp]
  \begin{scriptsize}
    \caption{Comparison of the cut-CC method with and without lifting for maximum cycle length 4 and different chain lengths, for the FSE policy.}
    \label{tab:aggrlifting_cyc4-method1-policy2}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrr@{}}\toprule
       & \multicolumn{4}{c}{with lifting} & \multicolumn{4}{c}{without lifting}\\
      \cmidrule{2-5} \cmidrule{6-9}
      \#vertices & \#opt & time & \#att. & \#sub & \#opt & time & \#att. & \#sub \\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 2}\\
       20 &  120 & 1.7 & 3.8 & 12.8 &  120 & 1.8 & 3.9 & 18.1\\
       50 &  62 & 1190.3 & 10.9 & 96.8 &  57 & 1394.2 & 10.7 & 167.4\\
      100 &  3 & 3548.7 & 1.4 & 6.0 &  2 & 3570.4 & 1.6 & 6.9\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 3}\\
       20 &  120 & 3.0 & 4.1 & 15.0 &  120 & 3.0 & 4.1 & 19.4\\
       50 &  50 & 1762.1 & 10.6 & 104.4 &  50 & 1809.0 & 9.8 & 118.3\\
      100 &  0 & 3600.0 & 0.0 & 0.0 &  0 & 3600.0 & 0.0 & 0.0\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 4}\\
       20 &  120 & 5.9 & 4.1 & 15.3 &  120 & 6.1 & 4.2 & 21.4\\
       50 &  21 & 2835.6 & 8.5 & 45.2 &  19 & 2953.9 & 9.6 & 82.2\\
      100 &  0 & 3600.0 & 0.0 & 0.0 &  0 & 3600.0 & 0.0 & 0.0\\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{table}


==> Tables/AggregatedLifting/aggr_lifting_table-cyc4-method2-policy1.tex <==
% generated by paper_generate_aggr_lifting_table.sh 4 s p 1
\begin{table}[htbp]
  \begin{scriptsize}
    \caption{Comparison of the cut-PICEF method with and without lifting for maximum cycle length 4 and different chain lengths, for the Full Recourse policy.}
    \label{tab:aggrlifting_cyc4-method2-policy1}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrr@{}}\toprule
       & \multicolumn{4}{c}{with lifting} & \multicolumn{4}{c}{without lifting}\\
      \cmidrule{2-5} \cmidrule{6-9}
      \#vertices & \#opt & time & \#att. & \#sub & \#opt & time & \#att. & \#sub \\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 2}\\
       20 &  120 & 0.3 & 2.8 & 8.8 &  120 & 0.4 & 2.9 & 12.5\\
       50 &  120 & 43.0 & 5.3 & 41.3 &  117 & 99.1 & 5.5 & 142.2\\
      100 &  73 & 1765.0 & 5.1 & 54.3 &  48 & 2475.0 & 8.4 & 342.4\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 3}\\
       20 &  120 & 0.6 & 2.9 & 8.7 &  120 & 0.6 & 3.0 & 11.8\\
       50 &  120 & 78.0 & 5.2 & 42.9 &  116 & 140.7 & 5.5 & 138.7\\
      100 &  68 & 2024.3 & 5.3 & 55.2 &  40 & 2755.4 & 4.6 & 96.9\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 4}\\
       20 &  120 & 0.8 & 3.0 & 8.9 &  120 & 0.7 & 3.0 & 12.3\\
       50 &  120 & 120.3 & 5.3 & 45.8 &  116 & 217.3 & 5.4 & 149.8\\
      100 &  66 & 2168.4 & 5.0 & 56.9 &  32 & 2886.3 & 4.3 & 118.2\\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{table}


==> Tables/AggregatedLifting/aggr_lifting_table-cyc4-method2-policy2.tex <==
% generated by paper_generate_aggr_lifting_table.sh 4 s p 2
\begin{table}[htbp]
  \begin{scriptsize}
    \caption{Comparison of the cut-PICEF method with and without lifting for maximum cycle length 4 and different chain lengths, for the FSE policy.}
    \label{tab:aggrlifting_cyc4-method2-policy2}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrr@{}}\toprule
       & \multicolumn{4}{c}{with lifting} & \multicolumn{4}{c}{without lifting}\\
      \cmidrule{2-5} \cmidrule{6-9}
      \#vertices & \#opt & time & \#att. & \#sub & \#opt & time & \#att. & \#sub \\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 2}\\
       20 &  120 & 2.0 & 3.7 & 12.4 &  120 & 1.9 & 3.9 & 19.9\\
       50 &  53 & 1383.8 & 10.1 & 83.2 &  56 & 1342.4 & 9.6 & 180.9\\
      100 &  2 & 3500.7 & 1.0 & 3.6 &  3 & 3573.6 & 1.6 & 7.4\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 3}\\
       20 &  120 & 3.2 & 3.7 & 12.5 &  120 & 3.2 & 3.8 & 18.5\\
       50 &  46 & 1921.2 & 10.0 & 76.6 &  44 & 1803.2 & 8.8 & 116.8\\
      100 &  1 & 3569.5 & 1.0 & 5.5 &  2 & 3561.2 & 1.1 & 4.8\\
      \midrule
      \multicolumn{9}{@{}l}{chain length: 4}\\
       20 &  120 & 4.0 & 4.0 & 15.2 &  120 & 3.9 & 4.0 & 21.9\\
       50 &  38 & 2143.5 & 8.8 & 58.0 &  36 & 2133.8 & 8.4 & 102.2\\
      100 &  1 & 3592.6 & 1.2 & 8.0 &  1 & 3588.7 & 1.2 & 9.2\\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{table}


==> Tables/LiftingTables/lifting_table-cyc3-method1-policy1.tex <==
% generated by paper_generate_lifting_table.sh 3 s c 1
\begin{sidewaystable}
  \begin{scriptsize}
    \caption{Comparison of the cut-CC method with and without lifting for maximum cycle length 3 and different chain lengths, for the Full Recourse policy.}
    \label{tab:lifting-cyc3-method1-policy1}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrrrrrr@{}}\toprule
       & \multicolumn{6}{c}{with lifting} & \multicolumn{6}{c}{without lifting}\\
      \cmidrule{2-7} \cmidrule{8-13}
      & & \multicolumn{3}{c}{time} & & & & \multicolumn{3}{c}{time} & & \\
      \cmidrule{3-5} \cmidrule{9-11}
      \#vertices & \#opt & total & stage 2 & stage 3 & \#att. & \#sub & \#opt & total & stage 2 & stage 3 & \#att. & \#sub \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 2}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.08} & \SI{12.23}{\percent} & \SI{19.22}{\percent} & \num{ 2.0} & \num{ 6.1}  &  \num{ 30} & \num{ 0.08} & \SI{15.67}{\percent} & \SI{19.56}{\percent} & \num{ 2.0} & \num{ 6.5} \\
       50 &  \num{ 30} & \num{ 2.86} & \SI{11.39}{\percent} & \SI{17.02}{\percent} & \num{ 3.5} & \num{ 15.6}  &  \num{ 30} & \num{ 2.88} & \SI{12.40}{\percent} & \SI{20.81}{\percent} & \num{ 3.4} & \num{ 17.1} \\
      100 &  \num{ 30} & \num{ 33.27} & \SI{7.13}{\percent} & \SI{17.38}{\percent} & \num{ 3.4} & \num{ 20.8}  &  \num{ 30} & \num{ 37.47} & \SI{7.98}{\percent} & \SI{25.18}{\percent} & \num{ 3.4} & \num{ 28.7} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.12} & \SI{24.86}{\percent} & \SI{15.43}{\percent} & \num{ 3.0} & \num{ 8.3}  &  \num{ 30} & \num{ 0.15} & \SI{30.15}{\percent} & \SI{16.11}{\percent} & \num{ 3.0} & \num{ 10.8} \\
       50 &  \num{ 30} & \num{ 4.88} & \SI{20.36}{\percent} & \SI{17.18}{\percent} & \num{ 4.5} & \num{ 29.3}  &  \num{ 30} & \num{ 8.42} & \SI{26.77}{\percent} & \SI{22.21}{\percent} & \num{ 4.8} & \num{ 60.8} \\
      100 &  \num{ 30} & \num{ 74.27} & \SI{9.13}{\percent} & \SI{19.33}{\percent} & \num{ 5.3} & \num{ 57.2}  &  \num{ 30} & \num{ 102.18} & \SI{19.79}{\percent} & \SI{30.22}{\percent} & \num{ 4.9} & \num{ 119.5} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.14} & \SI{32.30}{\percent} & \SI{13.57}{\percent} & \num{ 3.1} & \num{ 8.8}  &  \num{ 30} & \num{ 0.18} & \SI{28.96}{\percent} & \SI{16.26}{\percent} & \num{ 3.2} & \num{ 10.9} \\
       50 &  \num{ 30} & \num{ 8.78} & \SI{29.43}{\percent} & \SI{14.35}{\percent} & \num{ 5.9} & \num{ 48.5}  &  \num{ 30} & \num{ 17.82} & \SI{39.87}{\percent} & \SI{17.06}{\percent} & \num{ 6.1} & \num{ 126.6} \\
      100 &  \num{ 30} & \num{ 163.37} & \SI{20.28}{\percent} & \SI{23.41}{\percent} & \num{ 6.1} & \num{ 124.5}  &  \num{ 26} & \num{ 396.43} & \SI{37.39}{\percent} & \SI{28.33}{\percent} & \num{ 6.4} & \num{ 308.8} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.15} & \SI{37.16}{\percent} & \SI{15.66}{\percent} & \num{ 3.2} & \num{ 8.7}  &  \num{ 30} & \num{ 0.17} & \SI{32.37}{\percent} & \SI{14.32}{\percent} & \num{ 3.7} & \num{ 11.8} \\
       50 &  \num{ 30} & \num{ 12.63} & \SI{36.87}{\percent} & \SI{13.29}{\percent} & \num{ 6.7} & \num{ 73.2}  &  \num{ 30} & \num{ 42.06} & \SI{61.14}{\percent} & \SI{13.83}{\percent} & \num{ 6.9} & \num{ 248.0} \\
      100 &  \num{ 30} & \num{ 258.16} & \SI{28.08}{\percent} & \SI{21.96}{\percent} & \num{ 7.5} & \num{ 215.3}  &  \num{ 21} & \num{ 783.06} & \SI{50.85}{\percent} & \SI{19.76}{\percent} & \num{ 7.9} & \num{ 411.7} \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 3}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.17} & \SI{24.15}{\percent} & \SI{14.86}{\percent} & \num{ 2.0} & \num{ 6.2}  &  \num{ 30} & \num{ 0.17} & \SI{25.70}{\percent} & \SI{16.20}{\percent} & \num{ 2.0} & \num{ 6.3} \\
       50 &  \num{ 30} & \num{ 13.47} & \SI{8.23}{\percent} & \SI{15.36}{\percent} & \num{ 3.2} & \num{ 15.2}  &  \num{ 30} & \num{ 14.81} & \SI{8.78}{\percent} & \SI{19.01}{\percent} & \num{ 3.3} & \num{ 18.9} \\
      100 &  \num{ 28} & \num{ 540.66} & \SI{5.82}{\percent} & \SI{21.28}{\percent} & \num{ 3.7} & \num{ 26.6}  &  \num{ 25} & \num{ 597.63} & \SI{6.26}{\percent} & \SI{28.83}{\percent} & \num{ 3.5} & \num{ 33.0} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.23} & \SI{24.47}{\percent} & \SI{14.67}{\percent} & \num{ 2.8} & \num{ 9.9}  &  \num{ 30} & \num{ 0.28} & \SI{30.41}{\percent} & \SI{17.93}{\percent} & \num{ 2.8} & \num{ 13.1} \\
       50 &  \num{ 30} & \num{ 26.99} & \SI{12.72}{\percent} & \SI{15.56}{\percent} & \num{ 5.1} & \num{ 36.7}  &  \num{ 30} & \num{ 32.13} & \SI{16.95}{\percent} & \SI{23.45}{\percent} & \num{ 5.1} & \num{ 68.2} \\
      100 &  \num{ 23} & \num{1175.08} & \SI{5.42}{\percent} & \SI{21.29}{\percent} & \num{ 5.4} & \num{ 55.8}  &  \num{ 18} & \num{1415.26} & \SI{6.39}{\percent} & \SI{27.47}{\percent} & \num{ 5.9} & \num{ 89.3} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.31} & \SI{28.93}{\percent} & \SI{15.23}{\percent} & \num{ 3.3} & \num{ 8.8}  &  \num{ 30} & \num{ 0.43} & \SI{27.18}{\percent} & \SI{12.65}{\percent} & \num{ 3.6} & \num{ 12.7} \\
       50 &  \num{ 30} & \num{ 35.66} & \SI{15.54}{\percent} & \SI{13.38}{\percent} & \num{ 6.3} & \num{ 53.4}  &  \num{ 30} & \num{ 52.07} & \SI{30.26}{\percent} & \SI{22.88}{\percent} & \num{ 6.2} & \num{ 153.4} \\
      100 &  \num{ 20} & \num{1660.15} & \SI{7.33}{\percent} & \SI{28.94}{\percent} & \num{ 6.2} & \num{ 130.2}  &  \num{ 11} & \num{2093.21} & \SI{10.21}{\percent} & \SI{41.77}{\percent} & \num{ 5.7} & \num{ 200.7} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.22} & \SI{45.21}{\percent} & \SI{8.47}{\percent} & \num{ 3.0} & \num{ 8.7}  &  \num{ 30} & \num{ 0.20} & \SI{29.54}{\percent} & \SI{13.61}{\percent} & \num{ 3.4} & \num{ 11.2} \\
       50 &  \num{ 30} & \num{ 42.11} & \SI{21.59}{\percent} & \SI{14.25}{\percent} & \num{ 6.9} & \num{ 76.3}  &  \num{ 29} & \num{ 103.31} & \SI{42.99}{\percent} & \SI{18.11}{\percent} & \num{ 7.2} & \num{ 265.9} \\
      100 &  \num{ 17} & \num{2155.48} & \SI{6.32}{\percent} & \SI{20.18}{\percent} & \num{ 8.1} & \num{ 181.9}  &  \num{ 6} & \num{2956.89} & \SI{15.72}{\percent} & \SI{33.07}{\percent} & \num{ 8.3} & \num{ 540.0} \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 4}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.57} & \SI{27.88}{\percent} & \SI{7.81}{\percent} & \num{ 2.1} & \num{ 5.8}  &  \num{ 30} & \num{ 0.58} & \SI{24.81}{\percent} & \SI{11.99}{\percent} & \num{ 2.1} & \num{ 6.2} \\
       50 &  \num{ 30} & \num{ 176.58} & \SI{5.27}{\percent} & \SI{12.19}{\percent} & \num{ 3.8} & \num{ 17.3}  &  \num{ 30} & \num{ 196.04} & \SI{5.21}{\percent} & \SI{17.33}{\percent} & \num{ 3.8} & \num{ 23.4} \\
      100 &  \num{ 3} & \num{3159.06} & \SI{10.15}{\percent} & \SI{4.91}{\percent} & \num{ 3.7} & \num{ 16.0}  &  \num{ 3} & \num{3283.32} & \SI{10.86}{\percent} & \SI{6.29}{\percent} & \num{ 3.7} & \num{ 34.3} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.89} & \SI{26.31}{\percent} & \SI{9.96}{\percent} & \num{ 3.0} & \num{ 10.6}  &  \num{ 30} & \num{ 0.91} & \SI{24.61}{\percent} & \SI{12.69}{\percent} & \num{ 2.8} & \num{ 13.5} \\
       50 &  \num{ 29} & \num{ 233.65} & \SI{7.81}{\percent} & \SI{17.87}{\percent} & \num{ 4.7} & \num{ 45.1}  &  \num{ 29} & \num{ 321.98} & \SI{10.08}{\percent} & \SI{29.94}{\percent} & \num{ 4.9} & \num{ 95.7} \\
      100 &  \num{ 2} & \num{3401.13} & \SI{8.40}{\percent} & \SI{7.42}{\percent} & \num{ 4.5} & \num{ 74.5}  &  \num{ 1} & \num{3477.83} & \SI{9.58}{\percent} & \SI{6.12}{\percent} & \num{ 7.0} & \num{ 56.0} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.93} & \SI{23.24}{\percent} & \SI{12.31}{\percent} & \num{ 3.1} & \num{ 8.8}  &  \num{ 30} & \num{ 0.90} & \SI{20.47}{\percent} & \SI{13.84}{\percent} & \num{ 3.2} & \num{ 12.4} \\
       50 &  \num{ 30} & \num{ 246.80} & \SI{9.82}{\percent} & \SI{17.30}{\percent} & \num{ 5.8} & \num{ 58.5}  &  \num{ 27} & \num{ 423.88} & \SI{15.23}{\percent} & \SI{27.43}{\percent} & \num{ 6.6} & \num{ 164.7} \\
      100 &  \num{ 2} & \num{3400.58} & \SI{5.16}{\percent} & \SI{5.91}{\percent} & \num{ 4.0} & \num{ 86.0}  &  \num{ 0} & \num{3600.00} & \SI{4.71}{\percent} & \SI{5.72}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.91} & \SI{26.08}{\percent} & \SI{13.68}{\percent} & \num{ 3.5} & \num{ 10.2}  &  \num{ 30} & \num{ 0.84} & \SI{25.28}{\percent} & \SI{8.16}{\percent} & \num{ 3.6} & \num{ 13.3} \\
       50 &  \num{ 29} & \num{ 334.62} & \SI{10.57}{\percent} & \SI{16.40}{\percent} & \num{ 7.5} & \num{ 82.1}  &  \num{ 25} & \num{ 563.46} & \SI{22.20}{\percent} & \SI{25.68}{\percent} & \num{ 7.8} & \num{ 227.4} \\
      100 &  \num{ 1} & \num{3498.25} & \SI{4.75}{\percent} & \SI{1.70}{\percent} & \num{10.0} & \num{ 90.0}  &  \num{ 0} & \num{3600.00} & \SI{4.34}{\percent} & \SI{1.94}{\percent} & --- & --- \\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{sidewaystable}


==> Tables/LiftingTables/lifting_table-cyc3-method1-policy2.tex <==
% generated by paper_generate_lifting_table.sh 3 s c 2
\begin{sidewaystable}
  \begin{scriptsize}
    \caption{Comparison of the cut-CC method with and without lifting for maximum cycle length 3 and different chain lengths, for the FSE policy.}
    \label{tab:lifting-cyc3-method1-policy2}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrrrrrr@{}}\toprule
       & \multicolumn{6}{c}{with lifting} & \multicolumn{6}{c}{without lifting}\\
      \cmidrule{2-7} \cmidrule{8-13}
      & & \multicolumn{3}{c}{time} & & & & \multicolumn{3}{c}{time} & & \\
      \cmidrule{3-5} \cmidrule{9-11}
      \#vertices & \#opt & total & stage 2 & stage 3 & \#att. & \#sub & \#opt & total & stage 2 & stage 3 & \#att. & \#sub \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 2}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.24} & \SI{28.59}{\percent} & \SI{12.25}{\percent} & \num{ 2.6} & \num{ 6.1}  &  \num{ 30} & \num{ 0.24} & \SI{31.49}{\percent} & \SI{4.67}{\percent} & \num{ 2.6} & \num{ 6.1} \\
       50 &  \num{ 30} & \num{ 8.19} & \SI{28.02}{\percent} & \SI{1.48}{\percent} & \num{ 5.2} & \num{ 16.7}  &  \num{ 30} & \num{ 8.23} & \SI{28.81}{\percent} & \SI{1.50}{\percent} & \num{ 5.2} & \num{ 17.0} \\
      100 &  \num{ 26} & \num{ 189.69} & \SI{30.38}{\percent} & \SI{0.60}{\percent} & \num{ 6.5} & \num{ 22.7}  &  \num{ 26} & \num{ 187.88} & \SI{30.48}{\percent} & \SI{0.54}{\percent} & \num{ 6.5} & \num{ 22.8} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.66} & \SI{33.63}{\percent} & \SI{8.70}{\percent} & \num{ 3.7} & \num{ 9.7}  &  \num{ 30} & \num{ 0.55} & \SI{33.79}{\percent} & \SI{10.00}{\percent} & \num{ 3.6} & \num{ 11.3} \\
       50 &  \num{ 29} & \num{ 45.46} & \SI{15.58}{\percent} & \SI{1.58}{\percent} & \num{ 9.2} & \num{ 53.5}  &  \num{ 29} & \num{ 49.68} & \SI{17.26}{\percent} & \SI{1.72}{\percent} & \num{ 9.4} & \num{ 65.4} \\
      100 &  \num{ 12} & \num{1490.95} & \SI{3.97}{\percent} & \SI{0.52}{\percent} & \num{11.1} & \num{ 50.2}  &  \num{ 11} & \num{1733.28} & \SI{4.35}{\percent} & \SI{0.51}{\percent} & \num{11.3} & \num{ 102.7} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.72} & \SI{38.41}{\percent} & \SI{7.29}{\percent} & \num{ 3.8} & \num{ 12.2}  &  \num{ 30} & \num{ 1.00} & \SI{47.74}{\percent} & \SI{14.46}{\percent} & \num{ 3.8} & \num{ 19.0} \\
       50 &  \num{ 27} & \num{ 179.89} & \SI{17.89}{\percent} & \SI{1.38}{\percent} & \num{14.2} & \num{ 117.7}  &  \num{ 27} & \num{ 235.93} & \SI{23.44}{\percent} & \SI{1.60}{\percent} & \num{14.3} & \num{ 157.2} \\
      100 &  \num{ 6} & \num{2901.80} & \SI{5.41}{\percent} & \SI{0.42}{\percent} & \num{16.2} & \num{ 227.8}  &  \num{ 4} & \num{2808.18} & \SI{6.33}{\percent} & \SI{0.56}{\percent} & \num{14.5} & \num{ 159.0} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.47} & \SI{53.04}{\percent} & \SI{8.01}{\percent} & \num{ 3.4} & \num{ 9.0}  &  \num{ 30} & \num{ 0.35} & \SI{42.87}{\percent} & \SI{13.45}{\percent} & \num{ 3.6} & \num{ 10.8} \\
       50 &  \num{ 22} & \num{ 445.11} & \SI{20.75}{\percent} & \SI{1.12}{\percent} & \num{16.7} & \num{ 180.9}  &  \num{ 21} & \num{ 596.78} & \SI{28.85}{\percent} & \SI{1.54}{\percent} & \num{17.0} & \num{ 358.1} \\
      100 &  \num{ 1} & \num{3510.64} & \SI{2.65}{\percent} & \SI{0.23}{\percent} & \num{13.0} & \num{ 307.0}  &  \num{ 0} & \num{3600.00} & \SI{4.76}{\percent} & \SI{0.33}{\percent} & --- & --- \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 3}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.86} & \SI{32.10}{\percent} & \SI{7.62}{\percent} & \num{ 2.7} & \num{ 6.4}  &  \num{ 30} & \num{ 0.86} & \SI{35.61}{\percent} & \SI{5.26}{\percent} & \num{ 2.7} & \num{ 6.9} \\
       50 &  \num{ 28} & \num{ 94.78} & \SI{22.95}{\percent} & \SI{0.73}{\percent} & \num{ 5.5} & \num{ 19.5}  &  \num{ 28} & \num{ 98.70} & \SI{23.32}{\percent} & \SI{0.66}{\percent} & \num{ 5.6} & \num{ 21.0} \\
      100 &  \num{ 14} & \num{2132.62} & \SI{32.61}{\percent} & \SI{0.70}{\percent} & \num{ 5.6} & \num{ 20.1}  &  \num{ 13} & \num{2198.62} & \SI{32.36}{\percent} & \SI{0.69}{\percent} & \num{ 5.6} & \num{ 19.9} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 1.90} & \SI{39.55}{\percent} & \SI{4.70}{\percent} & \num{ 4.1} & \num{ 11.6}  &  \num{ 30} & \num{ 2.18} & \SI{31.51}{\percent} & \SI{11.82}{\percent} & \num{ 4.2} & \num{ 14.9} \\
       50 &  \num{ 24} & \num{ 298.22} & \SI{14.82}{\percent} & \SI{0.91}{\percent} & \num{ 8.8} & \num{ 53.5}  &  \num{ 24} & \num{ 330.08} & \SI{16.62}{\percent} & \SI{1.16}{\percent} & \num{ 8.9} & \num{ 63.8} \\
      100 &  \num{ 2} & \num{3546.73} & \SI{11.28}{\percent} & \SI{0.54}{\percent} & \num{17.5} & \num{ 84.0}  &  \num{ 2} & \num{3343.52} & \SI{9.90}{\percent} & \SI{0.54}{\percent} & \num{13.0} & \num{ 43.5} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 2.38} & \SI{43.71}{\percent} & \SI{14.70}{\percent} & \num{ 4.0} & \num{ 13.1}  &  \num{ 30} & \num{ 2.43} & \SI{41.52}{\percent} & \SI{14.90}{\percent} & \num{ 4.0} & \num{ 19.3} \\
       50 &  \num{ 17} & \num{ 768.87} & \SI{16.95}{\percent} & \SI{0.89}{\percent} & \num{11.4} & \num{ 90.9}  &  \num{ 17} & \num{1136.03} & \SI{20.11}{\percent} & \SI{1.05}{\percent} & \num{14.8} & \num{ 156.4} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{12.27}{\percent} & \SI{0.52}{\percent} & --- & ---  &  \num{ 2} & \num{3547.29} & \SI{12.34}{\percent} & \SI{0.57}{\percent} & \num{18.0} & \num{ 192.5} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 1.43} & \SI{43.26}{\percent} & \SI{5.86}{\percent} & \num{ 3.6} & \num{ 12.0}  &  \num{ 30} & \num{ 1.81} & \SI{49.86}{\percent} & \SI{6.00}{\percent} & \num{ 4.0} & \num{ 19.1} \\
       50 &  \num{ 11} & \num{1570.83} & \SI{20.73}{\percent} & \SI{0.75}{\percent} & \num{16.1} & \num{ 132.5}  &  \num{ 12} & \num{1491.58} & \SI{25.46}{\percent} & \SI{0.99}{\percent} & \num{15.2} & \num{ 209.5} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{9.51}{\percent} & \SI{0.19}{\percent} & --- & ---  &  \num{ 1} & \num{3518.60} & \SI{9.54}{\percent} & \SI{0.23}{\percent} & \num{14.0} & \num{ 192.0} \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 4}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 4.26} & \SI{21.76}{\percent} & \SI{8.68}{\percent} & \num{ 2.8} & \num{ 6.4}  &  \num{ 30} & \num{ 3.66} & \SI{36.13}{\percent} & \SI{4.14}{\percent} & \num{ 2.8} & \num{ 6.7} \\
       50 &  \num{ 19} & \num{ 683.29} & \SI{23.13}{\percent} & \SI{0.61}{\percent} & \num{ 4.7} & \num{ 14.3}  &  \num{ 20} & \num{ 692.00} & \SI{23.34}{\percent} & \SI{0.69}{\percent} & \num{ 4.7} & \num{ 14.7} \\
      100 &  \num{ 1} & \num{3561.68} & \SI{19.96}{\percent} & \SI{0.17}{\percent} & \num{ 6.0} & \num{ 20.0}  &  \num{ 1} & \num{3566.63} & \SI{18.65}{\percent} & \SI{0.13}{\percent} & \num{ 5.0} & \num{ 11.0} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 5.74} & \SI{38.40}{\percent} & \SI{8.26}{\percent} & \num{ 4.2} & \num{ 13.8}  &  \num{ 30} & \num{ 6.11} & \SI{30.63}{\percent} & \SI{10.35}{\percent} & \num{ 4.2} & \num{ 17.2} \\
       50 &  \num{ 8} & \num{1790.82} & \SI{12.98}{\percent} & \SI{0.52}{\percent} & \num{ 8.8} & \num{ 37.5}  &  \num{ 9} & \num{1655.99} & \SI{13.84}{\percent} & \SI{0.65}{\percent} & \num{ 8.3} & \num{ 39.1} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{12.39}{\percent} & \SI{0.05}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{12.00}{\percent} & \SI{0.06}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 5.78} & \SI{46.19}{\percent} & \SI{6.09}{\percent} & \num{ 4.4} & \num{ 14.6}  &  \num{ 30} & \num{ 4.81} & \SI{33.41}{\percent} & \SI{7.84}{\percent} & \num{ 3.9} & \num{ 16.1} \\
       50 &  \num{ 6} & \num{2095.81} & \SI{16.61}{\percent} & \SI{0.53}{\percent} & \num{11.8} & \num{ 73.8}  &  \num{ 6} & \num{2149.74} & \SI{15.14}{\percent} & \SI{0.54}{\percent} & \num{13.3} & \num{ 86.3} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{15.62}{\percent} & \SI{0.05}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{15.93}{\percent} & \SI{0.04}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 2.58} & \SI{40.08}{\percent} & \SI{5.65}{\percent} & \num{ 3.3} & \num{ 9.1}  &  \num{ 30} & \num{ 3.07} & \SI{45.49}{\percent} & \SI{6.24}{\percent} & \num{ 3.5} & \num{ 14.6} \\
       50 &  \num{ 4} & \num{2591.61} & \SI{17.44}{\percent} & \SI{0.38}{\percent} & \num{16.5} & \num{ 103.8}  &  \num{ 4} & \num{2640.83} & \SI{22.61}{\percent} & \SI{0.49}{\percent} & \num{17.8} & \num{ 133.0} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{17.94}{\percent} & \SI{0.04}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{17.15}{\percent} & \SI{0.05}{\percent} & --- & --- \\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{sidewaystable}


==> Tables/LiftingTables/lifting_table-cyc3-method2-policy1.tex <==
% generated by paper_generate_lifting_table.sh 3 s p 1
\begin{sidewaystable}
  \begin{scriptsize}
    \caption{Comparison of the cut-PICEF method with and without lifting for maximum cycle length 3 and different chain lengths, for the Full Recourse policy.}
    \label{tab:lifting-cyc3-method2-policy1}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrrrrrr@{}}\toprule
       & \multicolumn{6}{c}{with lifting} & \multicolumn{6}{c}{without lifting}\\
      \cmidrule{2-7} \cmidrule{8-13}
      & & \multicolumn{3}{c}{time} & & & & \multicolumn{3}{c}{time} & & \\
      \cmidrule{3-5} \cmidrule{9-11}
      \#vertices & \#opt & total & stage 2 & stage 3 & \#att. & \#sub & \#opt & total & stage 2 & stage 3 & \#att. & \#sub \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 2}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.11} & \SI{30.59}{\percent} & \SI{23.31}{\percent} & \num{ 1.9} & \num{ 5.9}  &  \num{ 30} & \num{ 0.08} & \SI{21.96}{\percent} & \SI{15.64}{\percent} & \num{ 1.9} & \num{ 6.1} \\
       50 &  \num{ 30} & \num{ 4.82} & \SI{16.41}{\percent} & \SI{38.36}{\percent} & \num{ 3.1} & \num{ 14.1}  &  \num{ 30} & \num{ 3.18} & \SI{11.68}{\percent} & \SI{22.63}{\percent} & \num{ 3.1} & \num{ 14.9} \\
      100 &  \num{ 30} & \num{ 62.88} & \SI{11.65}{\percent} & \SI{45.83}{\percent} & \num{ 3.3} & \num{ 21.7}  &  \num{ 30} & \num{ 43.32} & \SI{8.55}{\percent} & \SI{31.72}{\percent} & \num{ 3.6} & \num{ 31.1} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.16} & \SI{25.08}{\percent} & \SI{17.51}{\percent} & \num{ 2.7} & \num{ 8.3}  &  \num{ 30} & \num{ 0.16} & \SI{35.88}{\percent} & \SI{13.95}{\percent} & \num{ 2.6} & \num{ 10.4} \\
       50 &  \num{ 30} & \num{ 9.00} & \SI{17.96}{\percent} & \SI{35.47}{\percent} & \num{ 4.6} & \num{ 26.9}  &  \num{ 30} & \num{ 9.54} & \SI{26.18}{\percent} & \SI{19.87}{\percent} & \num{ 4.8} & \num{ 52.3} \\
      100 &  \num{ 30} & \num{ 152.87} & \SI{11.69}{\percent} & \SI{48.87}{\percent} & \num{ 5.3} & \num{ 57.1}  &  \num{ 30} & \num{ 137.89} & \SI{20.23}{\percent} & \SI{29.31}{\percent} & \num{ 5.5} & \num{ 120.2} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.16} & \SI{33.04}{\percent} & \SI{18.60}{\percent} & \num{ 3.1} & \num{ 8.5}  &  \num{ 30} & \num{ 0.16} & \SI{35.42}{\percent} & \SI{20.68}{\percent} & \num{ 3.0} & \num{ 10.8} \\
       50 &  \num{ 30} & \num{ 14.91} & \SI{25.84}{\percent} & \SI{32.99}{\percent} & \num{ 6.2} & \num{ 43.3}  &  \num{ 30} & \num{ 25.55} & \SI{48.76}{\percent} & \SI{16.67}{\percent} & \num{ 6.1} & \num{ 138.5} \\
      100 &  \num{ 30} & \num{ 319.64} & \SI{12.80}{\percent} & \SI{53.06}{\percent} & \num{ 6.4} & \num{ 94.5}  &  \num{ 25} & \num{ 518.40} & \SI{40.29}{\percent} & \SI{25.17}{\percent} & \num{ 7.2} & \num{ 247.8} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.21} & \SI{37.54}{\percent} & \SI{22.98}{\percent} & \num{ 3.3} & \num{ 9.0}  &  \num{ 30} & \num{ 0.13} & \SI{33.35}{\percent} & \SI{17.83}{\percent} & \num{ 3.4} & \num{ 10.0} \\
       50 &  \num{ 30} & \num{ 17.55} & \SI{27.70}{\percent} & \SI{34.28}{\percent} & \num{ 7.2} & \num{ 57.3}  &  \num{ 28} & \num{ 59.73} & \SI{57.61}{\percent} & \SI{10.67}{\percent} & \num{ 6.6} & \num{ 204.8} \\
      100 &  \num{ 29} & \num{ 542.21} & \SI{17.06}{\percent} & \SI{55.70}{\percent} & \num{ 7.8} & \num{ 166.0}  &  \num{ 18} & \num{1254.98} & \SI{59.81}{\percent} & \SI{19.31}{\percent} & \num{ 8.4} & \num{ 396.8} \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 3}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.21} & \SI{26.83}{\percent} & \SI{26.08}{\percent} & \num{ 1.8} & \num{ 5.7}  &  \num{ 30} & \num{ 0.14} & \SI{30.30}{\percent} & \SI{19.43}{\percent} & \num{ 1.8} & \num{ 5.7} \\
       50 &  \num{ 30} & \num{ 9.38} & \SI{16.25}{\percent} & \SI{39.86}{\percent} & \num{ 2.9} & \num{ 11.6}  &  \num{ 30} & \num{ 5.57} & \SI{10.35}{\percent} & \SI{29.30}{\percent} & \num{ 3.0} & \num{ 13.7} \\
      100 &  \num{ 30} & \num{ 119.61} & \SI{13.72}{\percent} & \SI{40.38}{\percent} & \num{ 3.9} & \num{ 22.8}  &  \num{ 30} & \num{ 114.01} & \SI{8.76}{\percent} & \SI{36.75}{\percent} & \num{ 4.0} & \num{ 30.8} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.36} & \SI{24.98}{\percent} & \SI{21.49}{\percent} & \num{ 2.8} & \num{ 8.9}  &  \num{ 30} & \num{ 0.31} & \SI{22.48}{\percent} & \SI{19.08}{\percent} & \num{ 2.8} & \num{ 11.0} \\
       50 &  \num{ 30} & \num{ 22.31} & \SI{16.54}{\percent} & \SI{47.45}{\percent} & \num{ 4.3} & \num{ 31.3}  &  \num{ 30} & \num{ 18.69} & \SI{17.94}{\percent} & \SI{34.13}{\percent} & \num{ 4.6} & \num{ 55.5} \\
      100 &  \num{ 30} & \num{ 244.16} & \SI{9.25}{\percent} & \SI{55.42}{\percent} & \num{ 4.6} & \num{ 56.7}  &  \num{ 29} & \num{ 303.46} & \SI{14.41}{\percent} & \SI{48.09}{\percent} & \num{ 4.9} & \num{ 120.0} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.28} & \SI{27.06}{\percent} & \SI{21.46}{\percent} & \num{ 3.1} & \num{ 7.8}  &  \num{ 30} & \num{ 0.28} & \SI{30.12}{\percent} & \SI{14.59}{\percent} & \num{ 3.1} & \num{ 11.1} \\
       50 &  \num{ 30} & \num{ 33.81} & \SI{19.32}{\percent} & \SI{47.81}{\percent} & \num{ 5.6} & \num{ 51.2}  &  \num{ 30} & \num{ 42.75} & \SI{35.71}{\percent} & \SI{28.34}{\percent} & \num{ 5.5} & \num{ 135.1} \\
      100 &  \num{ 27} & \num{ 752.24} & \SI{9.85}{\percent} & \SI{60.42}{\percent} & \num{ 6.4} & \num{ 95.8}  &  \num{ 21} & \num{1262.74} & \SI{25.70}{\percent} & \SI{54.60}{\percent} & \num{ 6.8} & \num{ 268.2} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.30} & \SI{40.42}{\percent} & \SI{16.63}{\percent} & \num{ 3.4} & \num{ 8.7}  &  \num{ 30} & \num{ 0.30} & \SI{38.98}{\percent} & \SI{10.52}{\percent} & \num{ 3.8} & \num{ 12.2} \\
       50 &  \num{ 30} & \num{ 44.07} & \SI{22.12}{\percent} & \SI{47.87}{\percent} & \num{ 6.6} & \num{ 69.0}  &  \num{ 28} & \num{ 75.70} & \SI{49.02}{\percent} & \SI{21.11}{\percent} & \num{ 7.4} & \num{ 185.8} \\
      100 &  \num{ 27} & \num{ 911.99} & \SI{10.91}{\percent} & \SI{59.01}{\percent} & \num{ 7.5} & \num{ 141.6}  &  \num{ 13} & \num{2140.89} & \SI{36.24}{\percent} & \SI{44.04}{\percent} & \num{ 8.9} & \num{ 364.5} \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 4}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.27} & \SI{32.80}{\percent} & \SI{21.78}{\percent} & \num{ 1.8} & \num{ 5.5}  &  \num{ 30} & \num{ 0.23} & \SI{24.25}{\percent} & \SI{23.81}{\percent} & \num{ 1.8} & \num{ 6.0} \\
       50 &  \num{ 30} & \num{ 19.20} & \SI{16.23}{\percent} & \SI{38.27}{\percent} & \num{ 3.1} & \num{ 12.7}  &  \num{ 30} & \num{ 16.06} & \SI{8.22}{\percent} & \SI{36.91}{\percent} & \num{ 3.1} & \num{ 18.5} \\
      100 &  \num{ 30} & \num{ 181.29} & \SI{10.58}{\percent} & \SI{49.64}{\percent} & \num{ 3.3} & \num{ 24.0}  &  \num{ 30} & \num{ 195.42} & \SI{7.60}{\percent} & \SI{53.41}{\percent} & \num{ 3.4} & \num{ 39.3} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.69} & \SI{31.50}{\percent} & \SI{21.52}{\percent} & \num{ 3.0} & \num{ 9.6}  &  \num{ 30} & \num{ 0.50} & \SI{24.01}{\percent} & \SI{12.87}{\percent} & \num{ 2.9} & \num{ 12.3} \\
       50 &  \num{ 30} & \num{ 40.93} & \SI{17.29}{\percent} & \SI{49.76}{\percent} & \num{ 4.3} & \num{ 35.4}  &  \num{ 30} & \num{ 41.36} & \SI{18.89}{\percent} & \SI{43.99}{\percent} & \num{ 4.2} & \num{ 77.2} \\
      100 &  \num{ 30} & \num{ 409.29} & \SI{8.86}{\percent} & \SI{46.99}{\percent} & \num{ 5.3} & \num{ 46.7}  &  \num{ 27} & \num{ 674.06} & \SI{14.31}{\percent} & \SI{56.58}{\percent} & \num{ 4.9} & \num{ 160.7} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.47} & \SI{26.41}{\percent} & \SI{25.16}{\percent} & \num{ 3.0} & \num{ 7.7}  &  \num{ 30} & \num{ 0.52} & \SI{37.43}{\percent} & \SI{13.49}{\percent} & \num{ 3.1} & \num{ 13.3} \\
       50 &  \num{ 30} & \num{ 63.96} & \SI{15.83}{\percent} & \SI{48.89}{\percent} & \num{ 5.7} & \num{ 51.6}  &  \num{ 30} & \num{ 79.13} & \SI{29.21}{\percent} & \SI{35.99}{\percent} & \num{ 6.0} & \num{ 153.9} \\
      100 &  \num{ 25} & \num{1165.20} & \SI{7.56}{\percent} & \SI{54.31}{\percent} & \num{ 6.6} & \num{ 83.9}  &  \num{ 18} & \num{1908.69} & \SI{21.57}{\percent} & \SI{58.79}{\percent} & \num{ 6.9} & \num{ 249.3} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.38} & \SI{27.85}{\percent} & \SI{21.63}{\percent} & \num{ 3.2} & \num{ 8.1}  &  \num{ 30} & \num{ 0.39} & \SI{28.25}{\percent} & \SI{16.86}{\percent} & \num{ 3.7} & \num{ 11.7} \\
       50 &  \num{ 30} & \num{ 70.60} & \SI{19.70}{\percent} & \SI{50.72}{\percent} & \num{ 6.7} & \num{ 72.4}  &  \num{ 27} & \num{ 134.69} & \SI{42.51}{\percent} & \SI{25.01}{\percent} & \num{ 7.2} & \num{ 193.7} \\
      100 &  \num{ 21} & \num{1525.97} & \SI{10.41}{\percent} & \SI{63.18}{\percent} & \num{ 7.3} & \num{ 115.1}  &  \num{ 6} & \num{3083.76} & \SI{32.60}{\percent} & \SI{50.54}{\percent} & \num{ 7.8} & \num{ 321.0} \\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{sidewaystable}


==> Tables/LiftingTables/lifting_table-cyc3-method2-policy2.tex <==
% generated by paper_generate_lifting_table.sh 3 s p 2
\begin{sidewaystable}
  \begin{scriptsize}
    \caption{Comparison of the cut-PICEF method with and without lifting for maximum cycle length 3 and different chain lengths, for the FSE policy.}
    \label{tab:lifting-cyc3-method2-policy2}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrrrrrr@{}}\toprule
       & \multicolumn{6}{c}{with lifting} & \multicolumn{6}{c}{without lifting}\\
      \cmidrule{2-7} \cmidrule{8-13}
      & & \multicolumn{3}{c}{time} & & & & \multicolumn{3}{c}{time} & & \\
      \cmidrule{3-5} \cmidrule{9-11}
      \#vertices & \#opt & total & stage 2 & stage 3 & \#att. & \#sub & \#opt & total & stage 2 & stage 3 & \#att. & \#sub \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 2}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.28} & \SI{18.49}{\percent} & \SI{5.94}{\percent} & \num{ 2.5} & \num{ 4.5}  &  \num{ 30} & \num{ 0.29} & \SI{13.69}{\percent} & \SI{10.64}{\percent} & \num{ 2.5} & \num{ 4.8} \\
       50 &  \num{ 29} & \num{ 31.19} & \SI{2.10}{\percent} & \SI{0.86}{\percent} & \num{ 4.4} & \num{ 11.2}  &  \num{ 29} & \num{ 33.57} & \SI{1.96}{\percent} & \SI{0.51}{\percent} & \num{ 4.5} & \num{ 10.6} \\
      100 &  \num{ 24} & \num{ 654.49} & \SI{0.36}{\percent} & \SI{0.11}{\percent} & \num{ 4.7} & \num{ 11.3}  &  \num{ 25} & \num{ 661.56} & \SI{0.34}{\percent} & \SI{0.05}{\percent} & \num{ 4.9} & \num{ 12.4} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.84} & \SI{27.50}{\percent} & \SI{5.53}{\percent} & \num{ 3.7} & \num{ 9.0}  &  \num{ 30} & \num{ 0.73} & \SI{17.90}{\percent} & \SI{10.76}{\percent} & \num{ 3.5} & \num{ 10.5} \\
       50 &  \num{ 27} & \num{ 134.12} & \SI{1.73}{\percent} & \SI{1.04}{\percent} & \num{ 8.0} & \num{ 33.7}  &  \num{ 27} & \num{ 125.42} & \SI{3.61}{\percent} & \SI{0.77}{\percent} & \num{ 8.1} & \num{ 41.9} \\
      100 &  \num{ 10} & \num{2199.59} & \SI{0.17}{\percent} & \SI{0.06}{\percent} & \num{ 6.8} & \num{ 23.1}  &  \num{ 9} & \num{2239.02} & \SI{0.15}{\percent} & \SI{0.05}{\percent} & \num{ 7.3} & \num{ 34.3} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.79} & \SI{34.29}{\percent} & \SI{8.95}{\percent} & \num{ 3.9} & \num{ 10.6}  &  \num{ 30} & \num{ 0.93} & \SI{24.09}{\percent} & \SI{15.57}{\percent} & \num{ 4.0} & \num{ 16.0} \\
       50 &  \num{ 21} & \num{ 438.07} & \SI{2.01}{\percent} & \SI{1.15}{\percent} & \num{11.5} & \num{ 59.3}  &  \num{ 22} & \num{ 401.65} & \SI{5.35}{\percent} & \SI{1.11}{\percent} & \num{11.3} & \num{ 91.6} \\
      100 &  \num{ 5} & \num{2765.90} & \SI{1.20}{\percent} & \SI{0.21}{\percent} & \num{ 8.4} & \num{ 176.6}  &  \num{ 2} & \num{3445.56} & \SI{0.10}{\percent} & \SI{2.59}{\percent} & \num{16.0} & \num{ 88.5} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.80} & \SI{28.26}{\percent} & \SI{13.92}{\percent} & \num{ 3.6} & \num{ 9.7}  &  \num{ 30} & \num{ 0.76} & \SI{38.74}{\percent} & \SI{13.75}{\percent} & \num{ 3.5} & \num{ 14.3} \\
       50 &  \num{ 18} & \num{ 892.46} & \SI{1.54}{\percent} & \SI{0.56}{\percent} & \num{16.1} & \num{ 107.7}  &  \num{ 17} & \num{ 830.07} & \SI{6.13}{\percent} & \SI{0.58}{\percent} & \num{15.3} & \num{ 185.9} \\
      100 &  \num{ 1} & \num{3568.64} & \SI{1.16}{\percent} & \SI{0.15}{\percent} & \num{ 7.0} & \num{ 68.0}  &  \num{ 0} & \num{3600.00} & \SI{0.09}{\percent} & \SI{0.03}{\percent} & --- & --- \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 3}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 1.61} & \SI{20.85}{\percent} & \SI{9.11}{\percent} & \num{ 2.9} & \num{ 5.6}  &  \num{ 30} & \num{ 1.50} & \SI{14.69}{\percent} & \SI{9.10}{\percent} & \num{ 2.9} & \num{ 5.8} \\
       50 &  \num{ 28} & \num{ 98.46} & \SI{0.95}{\percent} & \SI{0.34}{\percent} & \num{ 4.6} & \num{ 11.6}  &  \num{ 28} & \num{ 98.75} & \SI{0.94}{\percent} & \SI{0.15}{\percent} & \num{ 4.8} & \num{ 12.2} \\
      100 &  \num{ 15} & \num{1091.93} & \SI{0.40}{\percent} & \SI{0.06}{\percent} & \num{ 3.9} & \num{ 8.7}  &  \num{ 14} & \num{1169.76} & \SI{0.19}{\percent} & \SI{0.03}{\percent} & \num{ 3.9} & \num{ 8.6} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 1.94} & \SI{23.63}{\percent} & \SI{9.08}{\percent} & \num{ 3.8} & \num{ 10.4}  &  \num{ 30} & \num{ 1.87} & \SI{15.34}{\percent} & \SI{9.36}{\percent} & \num{ 3.8} & \num{ 12.4} \\
       50 &  \num{ 18} & \num{ 516.60} & \SI{1.10}{\percent} & \SI{0.88}{\percent} & \num{ 7.2} & \num{ 29.7}  &  \num{ 18} & \num{ 635.58} & \SI{1.04}{\percent} & \SI{0.32}{\percent} & \num{ 7.7} & \num{ 34.9} \\
      100 &  \num{ 1} & \num{3435.58} & \SI{0.08}{\percent} & \SI{0.06}{\percent} & \num{ 4.0} & \num{ 18.0}  &  \num{ 0} & \num{3600.00} & \SI{0.07}{\percent} & \SI{0.02}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 2.23} & \SI{28.42}{\percent} & \SI{12.95}{\percent} & \num{ 3.9} & \num{ 11.7}  &  \num{ 30} & \num{ 2.60} & \SI{24.62}{\percent} & \SI{8.35}{\percent} & \num{ 4.3} & \num{ 18.7} \\
       50 &  \num{ 12} & \num{1402.97} & \SI{0.38}{\percent} & \SI{0.27}{\percent} & \num{11.4} & \num{ 51.6}  &  \num{ 15} & \num{1210.16} & \SI{0.63}{\percent} & \SI{0.21}{\percent} & \num{11.3} & \num{ 85.6} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.07}{\percent} & \SI{0.06}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.06}{\percent} & \SI{0.02}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 1.65} & \SI{35.00}{\percent} & \SI{10.02}{\percent} & \num{ 3.7} & \num{ 11.4}  &  \num{ 30} & \num{ 1.04} & \SI{30.14}{\percent} & \SI{13.76}{\percent} & \num{ 3.3} & \num{ 14.0} \\
       50 &  \num{ 12} & \num{1491.41} & \SI{0.75}{\percent} & \SI{0.53}{\percent} & \num{14.8} & \num{ 77.2}  &  \num{ 12} & \num{1783.44} & \SI{0.71}{\percent} & \SI{0.23}{\percent} & \num{17.6} & \num{ 177.4} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.09}{\percent} & \SI{0.10}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.05}{\percent} & \SI{0.01}{\percent} & --- & --- \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 4}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 1.43} & \SI{14.71}{\percent} & \SI{8.88}{\percent} & \num{ 2.7} & \num{ 5.3}  &  \num{ 30} & \num{ 1.31} & \SI{11.75}{\percent} & \SI{5.58}{\percent} & \num{ 2.7} & \num{ 5.2} \\
       50 &  \num{ 23} & \num{ 211.33} & \SI{0.75}{\percent} & \SI{0.41}{\percent} & \num{ 4.3} & \num{ 9.1}  &  \num{ 23} & \num{ 210.85} & \SI{0.77}{\percent} & \SI{0.16}{\percent} & \num{ 4.3} & \num{ 9.5} \\
      100 &  \num{ 6} & \num{2415.62} & \SI{1.89}{\percent} & \SI{0.04}{\percent} & \num{ 4.0} & \num{ 9.0}  &  \num{ 6} & \num{2563.12} & \SI{0.07}{\percent} & \SI{0.01}{\percent} & \num{ 4.0} & \num{ 9.5} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 3.63} & \SI{19.27}{\percent} & \SI{9.13}{\percent} & \num{ 4.2} & \num{ 12.5}  &  \num{ 30} & \num{ 3.83} & \SI{17.52}{\percent} & \SI{7.20}{\percent} & \num{ 4.2} & \num{ 15.2} \\
       50 &  \num{ 13} & \num{ 984.53} & \SI{0.46}{\percent} & \SI{0.31}{\percent} & \num{ 6.8} & \num{ 30.4}  &  \num{ 15} & \num{ 968.64} & \SI{0.48}{\percent} & \SI{0.15}{\percent} & \num{ 7.0} & \num{ 39.4} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.07}{\percent} & \SI{0.04}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.04}{\percent} & \SI{0.01}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 2.90} & \SI{32.29}{\percent} & \SI{9.78}{\percent} & \num{ 4.3} & \num{ 13.9}  &  \num{ 30} & \num{ 3.67} & \SI{23.60}{\percent} & \SI{8.39}{\percent} & \num{ 4.6} & \num{ 23.0} \\
       50 &  \num{ 11} & \num{1388.61} & \SI{0.95}{\percent} & \SI{0.93}{\percent} & \num{10.7} & \num{ 73.5}  &  \num{ 9} & \num{1738.23} & \SI{0.70}{\percent} & \SI{0.11}{\percent} & \num{11.9} & \num{ 93.7} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.09}{\percent} & \SI{0.06}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.04}{\percent} & \SI{0.02}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 2.39} & \SI{26.15}{\percent} & \SI{9.82}{\percent} & \num{ 4.0} & \num{ 12.2}  &  \num{ 30} & \num{ 2.24} & \SI{25.68}{\percent} & \SI{15.86}{\percent} & \num{ 4.1} & \num{ 18.2} \\
       50 &  \num{ 7} & \num{1769.68} & \SI{0.58}{\percent} & \SI{1.19}{\percent} & \num{10.9} & \num{ 65.6}  &  \num{ 9} & \num{1896.04} & \SI{0.69}{\percent} & \SI{1.74}{\percent} & \num{14.2} & \num{ 120.2} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.12}{\percent} & \SI{0.06}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.04}{\percent} & \SI{0.02}{\percent} & --- & --- \\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{sidewaystable}


==> Tables/LiftingTables/lifting_table-cyc4-method1-policy1.tex <==
% generated by paper_generate_lifting_table.sh 4 s c 1
\begin{sidewaystable}
  \begin{scriptsize}
    \caption{Comparison of the cut-CC method with and without lifting for maximum cycle length 4 and different chain lengths, for the Full Recourse policy.}
    \label{tab:lifting-cyc4-method1-policy1}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrrrrrr@{}}\toprule
       & \multicolumn{6}{c}{with lifting} & \multicolumn{6}{c}{without lifting}\\
      \cmidrule{2-7} \cmidrule{8-13}
      & & \multicolumn{3}{c}{time} & & & & \multicolumn{3}{c}{time} & & \\
      \cmidrule{3-5} \cmidrule{9-11}
      \#vertices & \#opt & total & stage 2 & stage 3 & \#att. & \#sub & \#opt & total & stage 2 & stage 3 & \#att. & \#sub \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 2}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.15} & \SI{20.18}{\percent} & \SI{19.77}{\percent} & \num{ 1.8} & \num{ 6.7}  &  \num{ 30} & \num{ 0.15} & \SI{24.96}{\percent} & \SI{17.75}{\percent} & \num{ 1.8} & \num{ 7.7} \\
       50 &  \num{ 30} & \num{ 14.03} & \SI{7.32}{\percent} & \SI{18.81}{\percent} & \num{ 2.9} & \num{ 17.4}  &  \num{ 30} & \num{ 16.03} & \SI{8.32}{\percent} & \SI{26.97}{\percent} & \num{ 2.9} & \num{ 22.7} \\
      100 &  \num{ 28} & \num{ 591.86} & \SI{5.19}{\percent} & \SI{24.36}{\percent} & \num{ 3.4} & \num{ 25.0}  &  \num{ 26} & \num{ 893.61} & \SI{5.14}{\percent} & \SI{37.28}{\percent} & \num{ 3.5} & \num{ 45.3} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.30} & \SI{25.98}{\percent} & \SI{16.44}{\percent} & \num{ 3.0} & \num{ 10.9}  &  \num{ 30} & \num{ 0.40} & \SI{26.39}{\percent} & \SI{20.56}{\percent} & \num{ 2.9} & \num{ 15.2} \\
       50 &  \num{ 30} & \num{ 30.52} & \SI{13.02}{\percent} & \SI{14.77}{\percent} & \num{ 5.0} & \num{ 37.3}  &  \num{ 30} & \num{ 50.99} & \SI{25.07}{\percent} & \SI{27.72}{\percent} & \num{ 5.0} & \num{ 101.5} \\
      100 &  \num{ 23} & \num{1052.83} & \SI{5.88}{\percent} & \SI{25.35}{\percent} & \num{ 4.6} & \num{ 64.8}  &  \num{ 15} & \num{1904.66} & \SI{7.79}{\percent} & \SI{41.12}{\percent} & \num{ 4.9} & \num{ 147.7} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.29} & \SI{21.15}{\percent} & \SI{16.89}{\percent} & \num{ 3.2} & \num{ 8.4}  &  \num{ 30} & \num{ 0.55} & \SI{31.08}{\percent} & \SI{13.95}{\percent} & \num{ 3.6} & \num{ 16.1} \\
       50 &  \num{ 30} & \num{ 39.77} & \SI{17.47}{\percent} & \SI{13.85}{\percent} & \num{ 5.9} & \num{ 55.0}  &  \num{ 30} & \num{ 82.93} & \SI{38.76}{\percent} & \SI{22.90}{\percent} & \num{ 6.1} & \num{ 207.3} \\
      100 &  \num{ 15} & \num{1873.45} & \SI{5.75}{\percent} & \SI{20.20}{\percent} & \num{ 5.3} & \num{ 93.6}  &  \num{ 8} & \num{2972.21} & \SI{13.30}{\percent} & \SI{30.27}{\percent} & \num{ 5.9} & \num{ 333.6} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.31} & \SI{28.84}{\percent} & \SI{14.38}{\percent} & \num{ 3.4} & \num{ 9.4}  &  \num{ 30} & \num{ 0.38} & \SI{33.03}{\percent} & \SI{14.29}{\percent} & \num{ 3.3} & \num{ 12.9} \\
       50 &  \num{ 30} & \num{ 49.33} & \SI{17.86}{\percent} & \SI{11.72}{\percent} & \num{ 7.3} & \num{ 70.2}  &  \num{ 28} & \num{ 164.12} & \SI{50.80}{\percent} & \SI{15.87}{\percent} & \num{ 7.8} & \num{ 273.8} \\
      100 &  \num{ 17} & \num{1883.98} & \SI{7.87}{\percent} & \SI{21.47}{\percent} & \num{ 6.4} & \num{ 127.2}  &  \num{ 3} & \num{3410.61} & \SI{19.56}{\percent} & \SI{24.22}{\percent} & \num{ 9.0} & \num{ 534.7} \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 3}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.26} & \SI{20.60}{\percent} & \SI{12.48}{\percent} & \num{ 1.9} & \num{ 7.4}  &  \num{ 30} & \num{ 0.26} & \SI{27.11}{\percent} & \SI{13.20}{\percent} & \num{ 1.9} & \num{ 8.2} \\
       50 &  \num{ 30} & \num{ 31.68} & \SI{6.35}{\percent} & \SI{16.26}{\percent} & \num{ 2.9} & \num{ 18.1}  &  \num{ 30} & \num{ 37.67} & \SI{7.10}{\percent} & \SI{23.35}{\percent} & \num{ 3.1} & \num{ 24.5} \\
      100 &  \num{ 24} & \num{1182.61} & \SI{6.08}{\percent} & \SI{28.47}{\percent} & \num{ 3.0} & \num{ 27.2}  &  \num{ 21} & \num{1708.52} & \SI{6.25}{\percent} & \SI{44.78}{\percent} & \num{ 3.0} & \num{ 45.8} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.43} & \SI{27.36}{\percent} & \SI{17.40}{\percent} & \num{ 2.8} & \num{ 11.1}  &  \num{ 30} & \num{ 0.57} & \SI{32.87}{\percent} & \SI{13.25}{\percent} & \num{ 2.8} & \num{ 16.4} \\
       50 &  \num{ 30} & \num{ 60.41} & \SI{9.53}{\percent} & \SI{14.39}{\percent} & \num{ 4.7} & \num{ 36.1}  &  \num{ 30} & \num{ 100.92} & \SI{18.67}{\percent} & \SI{30.48}{\percent} & \num{ 4.8} & \num{ 114.1} \\
      100 &  \num{ 14} & \num{2350.91} & \SI{5.12}{\percent} & \SI{27.02}{\percent} & \num{ 4.5} & \num{ 68.4}  &  \num{ 7} & \num{3107.82} & \SI{5.38}{\percent} & \SI{29.00}{\percent} & \num{ 5.1} & \num{ 113.4} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.48} & \SI{20.53}{\percent} & \SI{12.22}{\percent} & \num{ 3.4} & \num{ 11.7}  &  \num{ 30} & \num{ 0.57} & \SI{28.76}{\percent} & \SI{15.65}{\percent} & \num{ 3.5} & \num{ 15.6} \\
       50 &  \num{ 30} & \num{ 80.68} & \SI{12.45}{\percent} & \SI{14.65}{\percent} & \num{ 5.9} & \num{ 62.9}  &  \num{ 30} & \num{ 180.85} & \SI{30.49}{\percent} & \SI{25.76}{\percent} & \num{ 6.3} & \num{ 225.0} \\
      100 &  \num{ 8} & \num{2934.43} & \SI{4.39}{\percent} & \SI{15.07}{\percent} & \num{ 5.4} & \num{ 81.6}  &  \num{ 1} & \num{3533.76} & \SI{5.03}{\percent} & \SI{22.44}{\percent} & \num{12.0} & \num{ 366.0} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.55} & \SI{33.89}{\percent} & \SI{8.00}{\percent} & \num{ 3.5} & \num{ 9.2}  &  \num{ 30} & \num{ 0.59} & \SI{26.99}{\percent} & \SI{11.21}{\percent} & \num{ 3.6} & \num{ 13.2} \\
       50 &  \num{ 30} & \num{ 111.86} & \SI{15.32}{\percent} & \SI{13.93}{\percent} & \num{ 7.1} & \num{ 90.5}  &  \num{ 27} & \num{ 228.29} & \SI{44.26}{\percent} & \SI{19.61}{\percent} & \num{ 6.9} & \num{ 286.0} \\
      100 &  \num{ 8} & \num{3092.19} & \SI{4.83}{\percent} & \SI{14.73}{\percent} & \num{ 6.4} & \num{ 120.6}  &  \num{ 1} & \num{3568.59} & \SI{6.95}{\percent} & \SI{17.52}{\percent} & \num{15.0} & \num{ 825.0} \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 4}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.69} & \SI{23.33}{\percent} & \SI{13.01}{\percent} & \num{ 2.0} & \num{ 7.5}  &  \num{ 30} & \num{ 0.69} & \SI{15.61}{\percent} & \SI{19.42}{\percent} & \num{ 2.0} & \num{ 8.6} \\
       50 &  \num{ 30} & \num{ 202.99} & \SI{4.96}{\percent} & \SI{14.72}{\percent} & \num{ 3.3} & \num{ 18.8}  &  \num{ 30} & \num{ 229.91} & \SI{5.72}{\percent} & \SI{23.29}{\percent} & \num{ 3.4} & \num{ 27.5} \\
      100 &  \num{ 3} & \num{3234.14} & \SI{10.12}{\percent} & \SI{8.90}{\percent} & \num{ 3.7} & \num{ 31.7}  &  \num{ 2} & \num{3327.35} & \SI{9.59}{\percent} & \SI{11.08}{\percent} & \num{ 3.0} & \num{ 55.5} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 1.12} & \SI{18.74}{\percent} & \SI{11.64}{\percent} & \num{ 3.0} & \num{ 11.6}  &  \num{ 30} & \num{ 1.13} & \SI{29.00}{\percent} & \SI{11.08}{\percent} & \num{ 2.9} & \num{ 16.4} \\
       50 &  \num{ 30} & \num{ 261.48} & \SI{6.83}{\percent} & \SI{16.13}{\percent} & \num{ 4.4} & \num{ 35.9}  &  \num{ 28} & \num{ 399.60} & \SI{11.82}{\percent} & \SI{33.90}{\percent} & \num{ 4.5} & \num{ 105.6} \\
      100 &  \num{ 3} & \num{3488.09} & \SI{9.02}{\percent} & \SI{8.46}{\percent} & \num{ 4.7} & \num{ 82.7}  &  \num{ 0} & \num{3600.00} & \SI{10.37}{\percent} & \SI{5.14}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.98} & \SI{15.67}{\percent} & \SI{12.82}{\percent} & \num{ 3.4} & \num{ 9.7}  &  \num{ 30} & \num{ 1.21} & \SI{24.97}{\percent} & \SI{12.50}{\percent} & \num{ 3.5} & \num{ 16.1} \\
       50 &  \num{ 27} & \num{ 396.12} & \SI{8.72}{\percent} & \SI{15.95}{\percent} & \num{ 5.6} & \num{ 65.7}  &  \num{ 24} & \num{ 686.29} & \SI{18.03}{\percent} & \SI{30.83}{\percent} & \num{ 6.2} & \num{ 197.5} \\
      100 &  \num{ 1} & \num{3541.42} & \SI{8.00}{\percent} & \SI{3.20}{\percent} & \num{ 7.0} & \num{ 122.0}  &  \num{ 0} & \num{3600.00} & \SI{9.87}{\percent} & \SI{1.76}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.91} & \SI{21.87}{\percent} & \SI{14.60}{\percent} & \num{ 3.4} & \num{ 9.2}  &  \num{ 30} & \num{ 0.93} & \SI{23.59}{\percent} & \SI{9.04}{\percent} & \num{ 3.3} & \num{ 13.8} \\
       50 &  \num{ 28} & \num{ 442.18} & \SI{8.24}{\percent} & \SI{13.60}{\percent} & \num{ 6.9} & \num{ 73.1}  &  \num{ 21} & \num{ 779.12} & \SI{23.65}{\percent} & \SI{26.43}{\percent} & \num{ 6.8} & \num{ 249.0} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{7.04}{\percent} & \SI{1.37}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{5.48}{\percent} & \SI{6.40}{\percent} & --- & --- \\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{sidewaystable}


==> Tables/LiftingTables/lifting_table-cyc4-method1-policy2.tex <==
% generated by paper_generate_lifting_table.sh 4 s c 2
\begin{sidewaystable}
  \begin{scriptsize}
    \caption{Comparison of the cut-CC method with and without lifting for maximum cycle length 4 and different chain lengths, for the FSE policy.}
    \label{tab:lifting-cyc4-method1-policy2}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrrrrrr@{}}\toprule
       & \multicolumn{6}{c}{with lifting} & \multicolumn{6}{c}{without lifting}\\
      \cmidrule{2-7} \cmidrule{8-13}
      & & \multicolumn{3}{c}{time} & & & & \multicolumn{3}{c}{time} & & \\
      \cmidrule{3-5} \cmidrule{9-11}
      \#vertices & \#opt & total & stage 2 & stage 3 & \#att. & \#sub & \#opt & total & stage 2 & stage 3 & \#att. & \#sub \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 2}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.99} & \SI{26.35}{\percent} & \SI{3.76}{\percent} & \num{ 3.0} & \num{ 7.3}  &  \num{ 30} & \num{ 0.99} & \SI{31.88}{\percent} & \SI{8.01}{\percent} & \num{ 3.0} & \num{ 7.9} \\
       50 &  \num{ 26} & \num{ 309.49} & \SI{11.79}{\percent} & \SI{0.45}{\percent} & \num{ 7.7} & \num{ 30.1}  &  \num{ 25} & \num{ 342.60} & \SI{11.85}{\percent} & \SI{0.51}{\percent} & \num{ 7.7} & \num{ 35.0} \\
      100 &  \num{ 3} & \num{3394.74} & \SI{21.92}{\percent} & \SI{0.37}{\percent} & \num{ 5.7} & \num{ 24.0}  &  \num{ 2} & \num{3481.47} & \SI{21.97}{\percent} & \SI{0.36}{\percent} & \num{ 6.5} & \num{ 27.5} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 2.92} & \SI{35.39}{\percent} & \SI{10.91}{\percent} & \num{ 4.6} & \num{ 17.8}  &  \num{ 30} & \num{ 2.83} & \SI{35.18}{\percent} & \SI{6.30}{\percent} & \num{ 4.3} & \num{ 21.4} \\
       50 &  \num{ 17} & \num{ 861.26} & \SI{11.54}{\percent} & \SI{0.63}{\percent} & \num{10.1} & \num{ 67.5}  &  \num{ 16} & \num{ 978.54} & \SI{14.67}{\percent} & \SI{0.83}{\percent} & \num{10.1} & \num{ 104.1} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{13.46}{\percent} & \SI{0.27}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{15.30}{\percent} & \SI{0.31}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 1.58} & \SI{43.50}{\percent} & \SI{14.44}{\percent} & \num{ 3.7} & \num{ 13.2}  &  \num{ 30} & \num{ 1.89} & \SI{48.14}{\percent} & \SI{6.34}{\percent} & \num{ 4.1} & \num{ 20.9} \\
       50 &  \num{ 12} & \num{1703.92} & \SI{18.40}{\percent} & \SI{0.61}{\percent} & \num{13.5} & \num{ 163.6}  &  \num{ 9} & \num{1983.83} & \SI{24.70}{\percent} & \SI{0.84}{\percent} & \num{10.9} & \num{ 226.3} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{13.77}{\percent} & \SI{0.18}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{15.24}{\percent} & \SI{0.21}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 1.24} & \SI{45.46}{\percent} & \SI{10.91}{\percent} & \num{ 3.7} & \num{ 12.9}  &  \num{ 30} & \num{ 1.46} & \SI{42.06}{\percent} & \SI{5.83}{\percent} & \num{ 4.1} & \num{ 22.2} \\
       50 &  \num{ 7} & \num{1886.33} & \SI{29.86}{\percent} & \SI{0.58}{\percent} & \num{12.3} & \num{ 125.9}  &  \num{ 7} & \num{2271.96} & \SI{40.37}{\percent} & \SI{0.91}{\percent} & \num{14.1} & \num{ 304.0} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{13.49}{\percent} & \SI{0.11}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{15.20}{\percent} & \SI{0.12}{\percent} & --- & --- \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 3}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 2.15} & \SI{27.42}{\percent} & \SI{4.61}{\percent} & \num{ 3.3} & \num{ 8.9}  &  \num{ 30} & \num{ 2.24} & \SI{28.40}{\percent} & \SI{8.36}{\percent} & \num{ 3.3} & \num{ 9.9} \\
       50 &  \num{ 23} & \num{ 560.38} & \SI{13.86}{\percent} & \SI{0.45}{\percent} & \num{ 6.7} & \num{ 26.8}  &  \num{ 25} & \num{ 525.96} & \SI{14.69}{\percent} & \SI{0.48}{\percent} & \num{ 7.1} & \num{ 30.0} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{32.83}{\percent} & \SI{0.45}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{32.01}{\percent} & \SI{0.38}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 3.93} & \SI{40.52}{\percent} & \SI{5.81}{\percent} & \num{ 5.0} & \num{ 18.1}  &  \num{ 30} & \num{ 4.10} & \SI{33.52}{\percent} & \SI{9.66}{\percent} & \num{ 4.9} & \num{ 21.5} \\
       50 &  \num{ 13} & \num{1576.63} & \SI{14.64}{\percent} & \SI{0.67}{\percent} & \num{ 9.5} & \num{ 78.0}  &  \num{ 12} & \num{1738.12} & \SI{16.03}{\percent} & \SI{0.69}{\percent} & \num{10.2} & \num{ 103.0} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{17.82}{\percent} & \SI{0.20}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{19.59}{\percent} & \SI{0.20}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 3.72} & \SI{46.18}{\percent} & \SI{7.65}{\percent} & \num{ 4.2} & \num{ 18.5}  &  \num{ 30} & \num{ 3.42} & \SI{43.68}{\percent} & \SI{15.84}{\percent} & \num{ 4.1} & \num{ 24.5} \\
       50 &  \num{ 9} & \num{2121.64} & \SI{22.54}{\percent} & \SI{0.57}{\percent} & \num{11.4} & \num{ 151.1}  &  \num{ 7} & \num{2464.55} & \SI{26.10}{\percent} & \SI{0.71}{\percent} & \num{11.1} & \num{ 183.3} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{19.97}{\percent} & \SI{0.14}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{21.03}{\percent} & \SI{0.16}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 2.40} & \SI{39.63}{\percent} & \SI{10.64}{\percent} & \num{ 4.1} & \num{ 14.5}  &  \num{ 30} & \num{ 2.27} & \SI{41.98}{\percent} & \SI{10.27}{\percent} & \num{ 4.1} & \num{ 21.7} \\
       50 &  \num{ 5} & \num{2789.68} & \SI{26.00}{\percent} & \SI{0.40}{\percent} & \num{14.8} & \num{ 161.6}  &  \num{ 6} & \num{2507.32} & \SI{35.23}{\percent} & \SI{0.67}{\percent} & \num{10.8} & \num{ 156.8} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{24.40}{\percent} & \SI{0.18}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{20.95}{\percent} & \SI{0.14}{\percent} & --- & --- \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 4}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 5.56} & \SI{25.03}{\percent} & \SI{2.70}{\percent} & \num{ 3.3} & \num{ 8.4}  &  \num{ 30} & \num{ 4.87} & \SI{31.53}{\percent} & \SI{4.27}{\percent} & \num{ 3.2} & \num{ 9.1} \\
       50 &  \num{ 14} & \num{1819.29} & \SI{18.32}{\percent} & \SI{0.57}{\percent} & \num{ 6.9} & \num{ 22.9}  &  \num{ 13} & \num{1749.18} & \SI{19.61}{\percent} & \SI{0.62}{\percent} & \num{ 6.9} & \num{ 23.6} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{27.36}{\percent} & \SI{0.17}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{25.56}{\percent} & \SI{0.18}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 7.96} & \SI{37.87}{\percent} & \SI{5.14}{\percent} & \num{ 5.0} & \num{ 19.3}  &  \num{ 30} & \num{ 8.64} & \SI{35.55}{\percent} & \SI{9.41}{\percent} & \num{ 5.2} & \num{ 25.0} \\
       50 &  \num{ 5} & \num{2849.70} & \SI{19.13}{\percent} & \SI{0.51}{\percent} & \num{ 9.2} & \num{ 45.8}  &  \num{ 3} & \num{3134.54} & \SI{17.63}{\percent} & \SI{0.55}{\percent} & \num{ 9.0} & \num{ 49.7} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{21.07}{\percent} & \SI{0.05}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{21.42}{\percent} & \SI{0.06}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 6.04} & \SI{36.62}{\percent} & \SI{9.95}{\percent} & \num{ 4.1} & \num{ 17.9}  &  \num{ 30} & \num{ 6.97} & \SI{43.25}{\percent} & \SI{9.94}{\percent} & \num{ 4.4} & \num{ 30.4} \\
       50 &  \num{ 1} & \num{3346.34} & \SI{21.33}{\percent} & \SI{0.43}{\percent} & \num{11.0} & \num{ 84.0}  &  \num{ 2} & \num{3431.51} & \SI{22.22}{\percent} & \SI{0.39}{\percent} & \num{11.5} & \num{ 113.5} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{23.64}{\percent} & \SI{0.06}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{22.95}{\percent} & \SI{0.06}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 3.88} & \SI{36.87}{\percent} & \SI{8.38}{\percent} & \num{ 4.0} & \num{ 15.7}  &  \num{ 30} & \num{ 3.77} & \SI{44.70}{\percent} & \SI{5.09}{\percent} & \num{ 4.0} & \num{ 21.3} \\
       50 &  \num{ 1} & \num{3326.92} & \SI{27.25}{\percent} & \SI{0.32}{\percent} & \num{ 7.0} & \num{ 28.0}  &  \num{ 1} & \num{3500.53} & \SI{32.45}{\percent} & \SI{0.40}{\percent} & \num{11.0} & \num{ 142.0} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{24.25}{\percent} & \SI{0.06}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{24.38}{\percent} & \SI{0.06}{\percent} & --- & --- \\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{sidewaystable}


==> Tables/LiftingTables/lifting_table-cyc4-method2-policy1.tex <==
% generated by paper_generate_lifting_table.sh 4 s p 1
\begin{sidewaystable}
  \begin{scriptsize}
    \caption{Comparison of the cut-PICEF method with and without lifting for maximum cycle length 4 and different chain lengths, for the Full Recourse policy.}
    \label{tab:lifting-cyc4-method2-policy1}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrrrrrr@{}}\toprule
       & \multicolumn{6}{c}{with lifting} & \multicolumn{6}{c}{without lifting}\\
      \cmidrule{2-7} \cmidrule{8-13}
      & & \multicolumn{3}{c}{time} & & & & \multicolumn{3}{c}{time} & & \\
      \cmidrule{3-5} \cmidrule{9-11}
      \#vertices & \#opt & total & stage 2 & stage 3 & \#att. & \#sub & \#opt & total & stage 2 & stage 3 & \#att. & \#sub \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 2}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.28} & \SI{14.36}{\percent} & \SI{17.24}{\percent} & \num{ 2.0} & \num{ 6.6}  &  \num{ 30} & \num{ 0.24} & \SI{16.77}{\percent} & \SI{24.50}{\percent} & \num{ 2.0} & \num{ 7.3} \\
       50 &  \num{ 30} & \num{ 21.30} & \SI{9.97}{\percent} & \SI{26.77}{\percent} & \num{ 3.1} & \num{ 15.5}  &  \num{ 30} & \num{ 18.13} & \SI{7.37}{\percent} & \SI{24.84}{\percent} & \num{ 3.0} & \num{ 21.2} \\
      100 &  \num{ 26} & \num{ 771.57} & \SI{7.97}{\percent} & \SI{35.34}{\percent} & \num{ 3.3} & \num{ 22.6}  &  \num{ 26} & \num{ 918.91} & \SI{5.62}{\percent} & \SI{43.40}{\percent} & \num{ 3.5} & \num{ 42.1} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.37} & \SI{23.44}{\percent} & \SI{18.82}{\percent} & \num{ 2.9} & \num{ 11.1}  &  \num{ 30} & \num{ 0.44} & \SI{23.22}{\percent} & \SI{16.24}{\percent} & \num{ 3.0} & \num{ 14.5} \\
       50 &  \num{ 30} & \num{ 41.73} & \SI{12.86}{\percent} & \SI{31.20}{\percent} & \num{ 4.9} & \num{ 34.8}  &  \num{ 30} & \num{ 51.56} & \SI{22.87}{\percent} & \SI{25.41}{\percent} & \num{ 5.0} & \num{ 79.8} \\
      100 &  \num{ 22} & \num{1284.22} & \SI{6.97}{\percent} & \SI{43.76}{\percent} & \num{ 4.5} & \num{ 50.4}  &  \num{ 15} & \num{2154.89} & \SI{8.62}{\percent} & \SI{44.55}{\percent} & \num{ 5.3} & \num{ 142.7} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.31} & \SI{32.27}{\percent} & \SI{15.51}{\percent} & \num{ 3.1} & \num{ 8.7}  &  \num{ 30} & \num{ 0.45} & \SI{34.28}{\percent} & \SI{19.87}{\percent} & \num{ 3.2} & \num{ 14.8} \\
       50 &  \num{ 30} & \num{ 45.70} & \SI{15.29}{\percent} & \SI{28.54}{\percent} & \num{ 5.9} & \num{ 43.2}  &  \num{ 30} & \num{ 139.06} & \SI{43.64}{\percent} & \SI{18.97}{\percent} & \num{ 6.4} & \num{ 240.4} \\
      100 &  \num{ 12} & \num{2539.34} & \SI{6.39}{\percent} & \SI{33.10}{\percent} & \num{ 6.1} & \num{ 62.3}  &  \num{ 6} & \num{3254.15} & \SI{11.60}{\percent} & \SI{38.67}{\percent} & \num{ 7.8} & \num{ 312.8} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.32} & \SI{35.11}{\percent} & \SI{21.44}{\percent} & \num{ 3.2} & \num{ 9.0}  &  \num{ 30} & \num{ 0.38} & \SI{36.45}{\percent} & \SI{15.05}{\percent} & \num{ 3.3} & \num{ 13.3} \\
       50 &  \num{ 30} & \num{ 63.38} & \SI{17.37}{\percent} & \SI{25.78}{\percent} & \num{ 7.3} & \num{ 71.8}  &  \num{ 27} & \num{ 187.50} & \SI{51.39}{\percent} & \SI{13.60}{\percent} & \num{ 7.6} & \num{ 227.5} \\
      100 &  \num{ 13} & \num{2464.68} & \SI{7.09}{\percent} & \SI{31.69}{\percent} & \num{ 6.5} & \num{ 81.8}  &  \num{ 1} & \num{3572.13} & \SI{16.26}{\percent} & \SI{25.13}{\percent} & \num{17.0} & \num{ 872.0} \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 3}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.38} & \SI{22.26}{\percent} & \SI{26.30}{\percent} & \num{ 1.9} & \num{ 6.5}  &  \num{ 30} & \num{ 0.35} & \SI{11.59}{\percent} & \SI{21.65}{\percent} & \num{ 1.9} & \num{ 7.4} \\
       50 &  \num{ 30} & \num{ 35.96} & \SI{11.25}{\percent} & \SI{36.59}{\percent} & \num{ 3.1} & \num{ 16.0}  &  \num{ 30} & \num{ 33.20} & \SI{7.30}{\percent} & \SI{35.49}{\percent} & \num{ 3.2} & \num{ 22.8} \\
      100 &  \num{ 25} & \num{ 785.72} & \SI{9.38}{\percent} & \SI{41.37}{\percent} & \num{ 3.1} & \num{ 23.0}  &  \num{ 27} & \num{1142.96} & \SI{6.47}{\percent} & \SI{52.07}{\percent} & \num{ 3.2} & \num{ 38.7} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.64} & \SI{28.77}{\percent} & \SI{20.95}{\percent} & \num{ 2.8} & \num{ 10.1}  &  \num{ 30} & \num{ 0.64} & \SI{27.73}{\percent} & \SI{17.01}{\percent} & \num{ 3.0} & \num{ 14.0} \\
       50 &  \num{ 30} & \num{ 78.94} & \SI{10.85}{\percent} & \SI{39.94}{\percent} & \num{ 4.9} & \num{ 35.5}  &  \num{ 30} & \num{ 98.34} & \SI{16.99}{\percent} & \SI{40.47}{\percent} & \num{ 5.0} & \num{ 90.1} \\
      100 &  \num{ 21} & \num{1847.92} & \SI{6.14}{\percent} & \SI{34.68}{\percent} & \num{ 5.3} & \num{ 50.9}  &  \num{ 10} & \num{2824.96} & \SI{6.82}{\percent} & \SI{48.93}{\percent} & \num{ 6.0} & \num{ 133.5} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.66} & \SI{25.48}{\percent} & \SI{16.31}{\percent} & \num{ 3.3} & \num{ 9.4}  &  \num{ 30} & \num{ 0.72} & \SI{28.46}{\percent} & \SI{16.55}{\percent} & \num{ 3.5} & \num{ 13.1} \\
       50 &  \num{ 30} & \num{ 90.92} & \SI{12.89}{\percent} & \SI{37.29}{\percent} & \num{ 5.9} & \num{ 52.2}  &  \num{ 29} & \num{ 169.80} & \SI{31.81}{\percent} & \SI{29.60}{\percent} & \num{ 6.3} & \num{ 195.4} \\
      100 &  \num{ 11} & \num{2722.26} & \SI{6.79}{\percent} & \SI{36.65}{\percent} & \num{ 6.5} & \num{ 60.5}  &  \num{ 3} & \num{3453.67} & \SI{9.41}{\percent} & \SI{46.40}{\percent} & \num{ 9.0} & \num{ 215.3} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.53} & \SI{26.14}{\percent} & \SI{13.74}{\percent} & \num{ 3.6} & \num{ 8.8}  &  \num{ 30} & \num{ 0.56} & \SI{31.99}{\percent} & \SI{16.11}{\percent} & \num{ 3.7} & \num{ 12.6} \\
       50 &  \num{ 30} & \num{ 106.01} & \SI{12.67}{\percent} & \SI{36.88}{\percent} & \num{ 7.1} & \num{ 67.8}  &  \num{ 27} & \num{ 261.47} & \SI{43.44}{\percent} & \SI{21.69}{\percent} & \num{ 7.4} & \num{ 246.6} \\
      100 &  \num{ 11} & \num{2741.17} & \SI{6.12}{\percent} & \SI{39.37}{\percent} & \num{ 6.2} & \num{ 86.4}  &  \num{ 0} & \num{3600.00} & \SI{11.48}{\percent} & \SI{42.81}{\percent} & --- & --- \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 4}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 0.63} & \SI{24.16}{\percent} & \SI{17.04}{\percent} & \num{ 2.1} & \num{ 6.6}  &  \num{ 30} & \num{ 0.56} & \SI{22.35}{\percent} & \SI{17.07}{\percent} & \num{ 2.1} & \num{ 7.3} \\
       50 &  \num{ 30} & \num{ 51.03} & \SI{10.70}{\percent} & \SI{38.72}{\percent} & \num{ 3.0} & \num{ 17.1}  &  \num{ 30} & \num{ 46.88} & \SI{7.09}{\percent} & \SI{39.38}{\percent} & \num{ 2.9} & \num{ 22.4} \\
      100 &  \num{ 26} & \num{ 951.26} & \SI{7.48}{\percent} & \SI{42.90}{\percent} & \num{ 2.6} & \num{ 23.2}  &  \num{ 24} & \num{1399.71} & \SI{5.73}{\percent} & \SI{60.70}{\percent} & \num{ 2.9} & \num{ 42.4} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 0.91} & \SI{23.25}{\percent} & \SI{23.76}{\percent} & \num{ 3.0} & \num{ 10.7}  &  \num{ 30} & \num{ 0.89} & \SI{29.88}{\percent} & \SI{15.96}{\percent} & \num{ 3.1} & \num{ 13.8} \\
       50 &  \num{ 30} & \num{ 100.21} & \SI{10.47}{\percent} & \SI{38.06}{\percent} & \num{ 4.7} & \num{ 34.1}  &  \num{ 30} & \num{ 156.36} & \SI{13.13}{\percent} & \SI{43.83}{\percent} & \num{ 5.1} & \num{ 97.3} \\
      100 &  \num{ 22} & \num{1770.23} & \SI{6.38}{\percent} & \SI{44.15}{\percent} & \num{ 4.4} & \num{ 50.1}  &  \num{ 7} & \num{2970.19} & \SI{6.55}{\percent} & \SI{52.23}{\percent} & \num{ 5.1} & \num{ 123.4} \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 0.72} & \SI{24.04}{\percent} & \SI{16.82}{\percent} & \num{ 3.3} & \num{ 9.1}  &  \num{ 30} & \num{ 0.76} & \SI{25.09}{\percent} & \SI{13.27}{\percent} & \num{ 3.6} & \num{ 15.6} \\
       50 &  \num{ 30} & \num{ 150.61} & \SI{10.95}{\percent} & \SI{35.87}{\percent} & \num{ 6.5} & \num{ 54.1}  &  \num{ 29} & \num{ 295.14} & \SI{28.06}{\percent} & \SI{35.31}{\percent} & \num{ 6.3} & \num{ 199.8} \\
      100 &  \num{ 8} & \num{2954.78} & \SI{6.64}{\percent} & \SI{37.47}{\percent} & \num{ 6.1} & \num{ 60.9}  &  \num{ 1} & \num{3575.11} & \SI{6.89}{\percent} & \SI{38.18}{\percent} & \num{ 9.0} & \num{ 307.0} \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 0.96} & \SI{31.95}{\percent} & \SI{16.48}{\percent} & \num{ 3.6} & \num{ 9.2}  &  \num{ 30} & \num{ 0.75} & \SI{32.61}{\percent} & \SI{10.70}{\percent} & \num{ 3.4} & \num{ 12.7} \\
       50 &  \num{ 30} & \num{ 179.42} & \SI{12.25}{\percent} & \SI{37.28}{\percent} & \num{ 7.1} & \num{ 77.8}  &  \num{ 27} & \num{ 370.75} & \SI{41.40}{\percent} & \SI{24.96}{\percent} & \num{ 7.3} & \num{ 279.9} \\
      100 &  \num{ 10} & \num{2997.36} & \SI{6.43}{\percent} & \SI{32.87}{\percent} & \num{ 6.8} & \num{ 93.5}  &  \num{ 0} & \num{3600.00} & \SI{10.26}{\percent} & \SI{36.56}{\percent} & --- & --- \\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{sidewaystable}


==> Tables/LiftingTables/lifting_table-cyc4-method2-policy2.tex <==
% generated by paper_generate_lifting_table.sh 4 s p 2
\begin{sidewaystable}
  \begin{scriptsize}
    \caption{Comparison of the cut-PICEF method with and without lifting for maximum cycle length 4 and different chain lengths, for the FSE policy.}
    \label{tab:lifting-cyc4-method2-policy2}
    \begin{tabular*}{\textwidth}{@{}l@{\;\;\extracolsep{\fill}}rrrrrrrrrrrr@{}}\toprule
       & \multicolumn{6}{c}{with lifting} & \multicolumn{6}{c}{without lifting}\\
      \cmidrule{2-7} \cmidrule{8-13}
      & & \multicolumn{3}{c}{time} & & & & \multicolumn{3}{c}{time} & & \\
      \cmidrule{3-5} \cmidrule{9-11}
      \#vertices & \#opt & total & stage 2 & stage 3 & \#att. & \#sub & \#opt & total & stage 2 & stage 3 & \#att. & \#sub \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 2}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 1.51} & \SI{15.56}{\percent} & \SI{12.12}{\percent} & \num{ 2.8} & \num{ 6.6}  &  \num{ 30} & \num{ 1.52} & \SI{16.23}{\percent} & \SI{12.21}{\percent} & \num{ 2.8} & \num{ 7.2} \\
       50 &  \num{ 25} & \num{ 416.08} & \SI{0.53}{\percent} & \SI{0.21}{\percent} & \num{ 6.1} & \num{ 21.9}  &  \num{ 23} & \num{ 425.01} & \SI{0.50}{\percent} & \SI{0.20}{\percent} & \num{ 5.7} & \num{ 19.5} \\
      100 &  \num{ 2} & \num{3202.94} & \SI{0.35}{\percent} & \SI{0.11}{\percent} & \num{ 4.0} & \num{ 14.5}  &  \num{ 3} & \num{3494.44} & \SI{0.32}{\percent} & \SI{0.11}{\percent} & \num{ 6.3} & \num{ 29.7} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 2.52} & \SI{29.67}{\percent} & \SI{4.92}{\percent} & \num{ 4.3} & \num{ 16.2}  &  \num{ 30} & \num{ 2.43} & \SI{20.22}{\percent} & \SI{8.33}{\percent} & \num{ 4.4} & \num{ 21.7} \\
       50 &  \num{ 13} & \num{1177.77} & \SI{1.04}{\percent} & \SI{0.49}{\percent} & \num{ 8.6} & \num{ 57.2}  &  \num{ 14} & \num{1235.50} & \SI{1.15}{\percent} & \SI{0.34}{\percent} & \num{ 9.1} & \num{ 89.9} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.36}{\percent} & \SI{0.13}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.34}{\percent} & \SI{0.10}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 2.29} & \SI{35.07}{\percent} & \SI{10.37}{\percent} & \num{ 3.8} & \num{ 14.7}  &  \num{ 30} & \num{ 2.30} & \SI{19.62}{\percent} & \SI{16.53}{\percent} & \num{ 4.3} & \num{ 30.6} \\
       50 &  \num{ 9} & \num{1608.00} & \SI{2.32}{\percent} & \SI{0.52}{\percent} & \num{ 9.7} & \num{ 99.8}  &  \num{ 11} & \num{1669.92} & \SI{5.09}{\percent} & \SI{0.70}{\percent} & \num{10.4} & \num{ 274.7} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.27}{\percent} & \SI{0.07}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.29}{\percent} & \SI{0.07}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 1.74} & \SI{27.38}{\percent} & \SI{15.88}{\percent} & \num{ 3.9} & \num{ 12.0}  &  \num{ 30} & \num{ 1.43} & \SI{21.99}{\percent} & \SI{9.85}{\percent} & \num{ 3.8} & \num{ 20.2} \\
       50 &  \num{ 6} & \num{2333.27} & \SI{1.24}{\percent} & \SI{0.36}{\percent} & \num{16.2} & \num{ 153.8}  &  \num{ 8} & \num{2039.06} & \SI{6.18}{\percent} & \SI{0.60}{\percent} & \num{13.4} & \num{ 339.6} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.29}{\percent} & \SI{0.07}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.33}{\percent} & \SI{0.10}{\percent} & --- & --- \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 3}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 1.85} & \SI{15.76}{\percent} & \SI{6.85}{\percent} & \num{ 2.8} & \num{ 6.9}  &  \num{ 30} & \num{ 1.90} & \SI{21.59}{\percent} & \SI{6.46}{\percent} & \num{ 2.8} & \num{ 7.8} \\
       50 &  \num{ 20} & \num{ 601.60} & \SI{0.34}{\percent} & \SI{0.18}{\percent} & \num{ 5.0} & \num{ 17.6}  &  \num{ 20} & \num{ 604.26} & \SI{0.34}{\percent} & \SI{0.13}{\percent} & \num{ 5.1} & \num{ 20.1} \\
      100 &  \num{ 1} & \num{3477.97} & \SI{0.30}{\percent} & \SI{0.09}{\percent} & \num{ 4.0} & \num{ 22.0}  &  \num{ 2} & \num{3444.94} & \SI{0.29}{\percent} & \SI{0.08}{\percent} & \num{ 4.5} & \num{ 19.0} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 4.71} & \SI{18.62}{\percent} & \SI{7.20}{\percent} & \num{ 4.6} & \num{ 16.4}  &  \num{ 30} & \num{ 4.54} & \SI{17.08}{\percent} & \SI{4.25}{\percent} & \num{ 4.7} & \num{ 19.9} \\
       50 &  \num{ 12} & \num{1993.30} & \SI{0.30}{\percent} & \SI{0.17}{\percent} & \num{ 9.8} & \num{ 64.4}  &  \num{ 11} & \num{2003.66} & \SI{0.37}{\percent} & \SI{0.11}{\percent} & \num{ 9.1} & \num{ 70.6} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.21}{\percent} & \SI{0.03}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.23}{\percent} & \SI{0.45}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 3.71} & \SI{38.58}{\percent} & \SI{5.60}{\percent} & \num{ 3.8} & \num{ 17.0}  &  \num{ 30} & \num{ 3.61} & \SI{24.62}{\percent} & \SI{8.44}{\percent} & \num{ 3.8} & \num{ 25.4} \\
       50 &  \num{ 8} & \num{2338.61} & \SI{0.55}{\percent} & \SI{0.27}{\percent} & \num{10.2} & \num{ 78.9}  &  \num{ 7} & \num{2326.23} & \SI{1.61}{\percent} & \SI{0.30}{\percent} & \num{10.1} & \num{ 197.4} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.23}{\percent} & \SI{0.05}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.22}{\percent} & \SI{0.03}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 2.44} & \SI{26.54}{\percent} & \SI{15.81}{\percent} & \num{ 3.4} & \num{ 9.5}  &  \num{ 30} & \num{ 2.83} & \SI{28.60}{\percent} & \SI{11.29}{\percent} & \num{ 4.0} & \num{ 20.7} \\
       50 &  \num{ 6} & \num{2751.21} & \SI{0.54}{\percent} & \SI{0.51}{\percent} & \num{14.8} & \num{ 145.7}  &  \num{ 6} & \num{2278.47} & \SI{1.28}{\percent} & \SI{0.43}{\percent} & \num{10.7} & \num{ 179.0} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.23}{\percent} & \SI{0.05}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.24}{\percent} & \SI{0.04}{\percent} & --- & --- \\
      \midrule
      \multicolumn{13}{@{}l}{chain length: 4}\\
      \multicolumn{13}{@{}l}{$B = 1$}\\
       20 &  \num{ 30} & \num{ 2.51} & \SI{19.56}{\percent} & \SI{7.74}{\percent} & \num{ 2.9} & \num{ 6.6}  &  \num{ 30} & \num{ 2.66} & \SI{18.13}{\percent} & \SI{6.05}{\percent} & \num{ 2.9} & \num{ 7.7} \\
       50 &  \num{ 18} & \num{1170.25} & \SI{0.19}{\percent} & \SI{0.09}{\percent} & \num{ 5.8} & \num{ 19.3}  &  \num{ 18} & \num{1105.75} & \SI{0.21}{\percent} & \SI{0.09}{\percent} & \num{ 5.6} & \num{ 20.4} \\
      100 &  \num{ 1} & \num{3570.22} & \SI{0.26}{\percent} & \SI{0.07}{\percent} & \num{ 5.0} & \num{ 32.0}  &  \num{ 1} & \num{3554.88} & \SI{0.24}{\percent} & \SI{0.05}{\percent} & \num{ 5.0} & \num{ 37.0} \\
      \multicolumn{13}{@{}l}{$B = 2$}\\
       20 &  \num{ 30} & \num{ 6.31} & \SI{21.15}{\percent} & \SI{6.59}{\percent} & \num{ 4.7} & \num{ 17.5}  &  \num{ 30} & \num{ 5.49} & \SI{18.03}{\percent} & \SI{8.23}{\percent} & \num{ 4.6} & \num{ 24.2} \\
       50 &  \num{ 8} & \num{2469.09} & \SI{0.23}{\percent} & \SI{0.27}{\percent} & \num{ 7.8} & \num{ 49.8}  &  \num{ 7} & \num{2561.70} & \SI{0.30}{\percent} & \SI{0.14}{\percent} & \num{ 8.0} & \num{ 82.9} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.29}{\percent} & \SI{0.15}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.28}{\percent} & \SI{0.10}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 3$}\\
       20 &  \num{ 30} & \num{ 4.39} & \SI{34.94}{\percent} & \SI{8.47}{\percent} & \num{ 4.5} & \num{ 22.1}  &  \num{ 30} & \num{ 5.01} & \SI{23.38}{\percent} & \SI{15.73}{\percent} & \num{ 4.6} & \num{ 36.2} \\
       50 &  \num{ 6} & \num{2301.26} & \SI{0.97}{\percent} & \SI{1.05}{\percent} & \num{ 8.2} & \num{ 49.2}  &  \num{ 6} & \num{2337.49} & \SI{0.46}{\percent} & \SI{0.24}{\percent} & \num{ 8.0} & \num{ 79.3} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.21}{\percent} & \SI{0.04}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.18}{\percent} & \SI{0.03}{\percent} & --- & --- \\
      \multicolumn{13}{@{}l}{$B = 4$}\\
       20 &  \num{ 30} & \num{ 2.82} & \SI{21.21}{\percent} & \SI{18.58}{\percent} & \num{ 3.9} & \num{ 14.4}  &  \num{ 30} & \num{ 2.48} & \SI{23.50}{\percent} & \SI{9.39}{\percent} & \num{ 3.9} & \num{ 19.4} \\
       50 &  \num{ 6} & \num{2633.30} & \SI{1.05}{\percent} & \SI{1.45}{\percent} & \num{13.5} & \num{ 114.0}  &  \num{ 5} & \num{2530.14} & \SI{2.42}{\percent} & \SI{0.76}{\percent} & \num{12.0} & \num{ 226.0} \\
      100 &  \num{ 0} & \num{3600.00} & \SI{0.28}{\percent} & \SI{0.07}{\percent} & --- & ---  &  \num{ 0} & \num{3600.00} & \SI{0.19}{\percent} & \SI{0.03}{\percent} & --- & --- \\
      \bottomrule
    \end{tabular*}
  \end{scriptsize}
\end{sidewaystable}

